Temporal Regular Path Queries

In the last decade, substantial progress has been made towards standardizing the syntax of graph query languages, and towards understanding their semantics and complexity of evaluation. In this paper, we consider temporal property graphs (TPGs) and propose temporal regular path queries (TRPQs) that incorporate time into TPG navigation. Starting with design principles, we propose a natural syntactic extension of the MATCH clause of popular graph query languages. We then formally present the semantics of TRPQs, and study the complexity of their evaluation. We show that TRPQs can be evaluated in polynomial time if TPGs are time-stamped with time points, and identify fragments of the TRPQ language that admit efficient evaluation over a more succinct interval-annotated representation. Finally, we implement a fragment of the language in a state-of-the-art dataflow framework, and experimentally demonstrate that TRPQ can be evaluated efficiently.

==> 6practgraph.tex <==
In the previous section, we showed that $\Lthree$ can be evaluated in polynomial time over TPGs in which time points are associated with nodes, edges, and properties.  This is an important positive result. However, time-stamping objects with time points may be impractical in terms of space overhead.   This motivates the development of interval-based representations, which are common for temporal models  for both relations (\eg ~\cite{DBLP:conf/sigmod/DignosBG12,Montanari2009}) and graphs (\eg ~\cite{DBLP:journals/tkde/ByunWK20,Debrouvier21,DBLP:conf/dbpl/MoffittS17}).  Point-based temporal semantics requires that representations be temporally coalesced: a pair of value-equivalent temporally adjacent tuples should be stored as a single tuple, and this property should be maintained through operations~\cite{DBLP:conf/vldb/BohlenSS96}.  

In this section, we formally define a succinct \tpg representation that uses interval time-stamping, which we call coalesced temporal property graph (\ctpg).  We study the complexity of the evaluation problem for \Lthree queries over \ctpgs. Importantly, this evaluation problem is much more challenging, as \ctpgs can be exponentially more succinct than \tpgs.

%In practice, extensively writing all time points of a \tg is undesirable, as the number of time points can be exponentially higher than the number of changes in the \tg across time. Instead, the notion of temporally-coalesced \tgs is used.

%Temporally-coalesced \tgs are succinct representations of \tgs that use intervals instead of time points. They allow a natural description of what changes throughout time in \tgs without explicitly declaring their state at each one of their time points.

% In this section, we will show why such representation is needed by linking property graphs, or \pgs, to temporal property graphs, or \tgs, through the concept of snapshots. This, in turn, will yield an interpretation of temporal regular path expressions when time is removed and an explanation to why \Lthree satisfies both backward compatibility and snapshot reducibility.

\subsection{Coalesced temporal property graphs}

%Recall that 
An interval of $\mathbb{N}$ is a term of the form $[a, b]$ with $a, b \in \N$ and $a \leq b$, which is used  as a concise representation of the set of natural numbers $\{i \in \N \ \vert \ a \leq i \leq b \}$ (that is, to specify this interval, we just need to mention its starting point $a$ and its ending point $b$). Using Allen's interval algebra~\cite{Allen1983}, given two intervals $[a_1,b_1]$ and $[a_2, b_2]$, we say that $[a_1, b_1]$ occurs during $[a_2, b_2]$ if $a_2 \leq a_1$ and $b_1 \leq b_2$, $[a_1, b_1]$ meets $[a_2, b_2]$ if $b_1 + 1 = b_2$, and $[a_1, b_1]$ is before $[a_2, b_2]$ if $b_1 + 1 < a_2$.   
%If $[a_1, b_1]$ meets $[a_2, b_2]$, we sometimes refer to such a pair of intervals as \emph{temporally-adjacent}.

A finite family $\F$ of intervals is said to be \emph{temporally coalesced}~\cite{DBLP:reference/db/Bohlen09}, or \emph{\coal} for short, if $\F = \{ [a_1, b_1], \ldots, [a_n, b_n] \}$ and $[a_j, b_j]$ is before $[a_{j+1}, b_{j+1}]$ for every $j \in \{1, \ldots, n-1\}$.   For example, $\F_1 = \{[1,4], [6,8]\}$ is \coal, while  $\F_2 = \{[1,2], [3,4], [6,8] \}$ is not, because $[1,2]$ meets $[3,4]$.
The set of all finite \coal families of intervals is denoted by $\fnc$.  Observe that $\emptyset \in \fnc$.
Moreover, given $\F_1, \F_2 \in \fnc$, family $\F_1$ is said to be contained in family $\F_2$, denoted by $\F_1 \sqsubseteq \F_2$, if for every $[a_1, b_1] \in \F_1$, there exists $[a_2, b_2] \in \F_2$ such that $[a_1, b_1]$ occurs during $[a_2, b_2]$. 
Finally, given an interval $\Omega$, we use $\fnc(\Omega)$ to denote the set of all families $\F \in \fnc$ such that for every $[a, b] \in \F$, it holds that $[a, b]$ occurs during $\Omega$.

Given an interval $[a, b]$ and $v \in \Val$, the pair $(v,[a, b])$ is a {\em valued} interval.  
A finite family $\F$ of valued intervals is said to be \coal if $\F = \{(v_1,[a_1, b_1])$, $\ldots$, $(v_n,[a_n, b_n])\}$ and for every $j \in \{1, \ldots, n-1\}$, either $[a_j, b_j]$ is before $[a_{j+1}, b_{j+1}]$, or $[a_j, b_j]$ meets $[a_{j+1}, b_{j+1}]$ and \mbox{$v_j \neq v_{j+1}$}.  For example, $\F_1 = \{(v, [1,2])$, $(v, [5,8]) \}$ and $\F_2 = \{(v, [1,2])$, $(w, [3,4]) \}$ are both \coal (assuming that $v \neq w$). On the other hand, $\F_3 = \{(v, [1,2])$, $(v, [3,4]) \}$ is not \coal because $[1,2]$ meets $[3,4]$ and these intervals have the same value in $\F_3$.
Moreover, the set of all finite \coal families of valued intervals is denoted by $\vfnc$.
Finally, given an interval $\Omega$, we use $\vfnc(\Omega)$ to denote the set of all families $\F \in \vfnc$ such that for every $(v,[a, b]) \in \F$, it holds that $[a, b]$ occurs during~$\Omega$. 

We finally have the necessary ingredients to introduce the notion of \coal temporal property graph.
\begin{definition}
\label{def:tg1}
\begin{sloppypar}
A 
%temporally-\coal \tg, or \coal \tg, for short, 
\coal temporal property graph (CTPG) is a tuple $\C = ( \Omega, N, E, \rho, \lambda, \xi, \sigma)$, where $N$, $E$, $\rho$ and $\lambda$ are defined exactly as for the case of TPGs (see Definition \ref{def:tg}). Moreover,
\end{sloppypar}
\begin{itemize}
%\setlength\itemsep{1pt}
\item $\Omega$ is an interval of $\mathbb{N}$;
\item $\xi: (N \cup E) \to \fnc(\Omega)$ is a function that maps a node or an edge to a finite \coal family of intervals occurring during $\Omega$;

\item $\sigma:  (N \cup E) \times \Prop \to \vfnc(\Omega)$ is a function that maps a node or an edge, and a property name to a finite \coal family of valued intervals occurring during $\Omega$.
\end{itemize}
%\setlength\itemsep{1pt}
In addition, $\C$ satisfies the following conditions:
\begin{itemize}
\item If $\rho(e) = (n_1,n_2)$, then  $\xi(e) \sqsubseteq \xi(n_1)$
and
$\xi(e) \sqsubseteq \xi(n_2)$.

\item 
%\begin{sloppypar}
There exists a finite set of pairs $(o,p) \in (N \cup E) \times \Prop$ such that $\sigma(o,p) \neq \emptyset$. Moreover, if $\sigma(o,p) = \{(v_1, [a_1, b_1])$, $\ldots$, $(v_n, [a_n, b_n])\}$, then $\{[a_1, b_1], \ldots, [a_n, b_n] \} \sqsubseteq \xi(o)$.\qed
%\end{sloppypar}
\end{itemize}
\end{definition}
%Observe that 
In the definition of a \ctpg, given a node or edge $o$, function $\xi$  indicates 
%for a node or edge $o$, 
the time intervals where $o$ exists,
%Given that $\xi(o)$ is a finite family of intervals, we have that $o$ exists only in a finite number of time points in $\N$. 
%Moreover, 
and function $\sigma$ indicates the values of a property $p$ for 
%a node or an edge 
$o$. More precisely, if $\sigma(o,p) = \{(v_1, [a_1, b_1]), \ldots, (v_n, [a_n, b_n])\}$, then the value of property $p$ for $o$ is $v_j$ in every time point in the interval $[a_j, b_j]$ ($1 \leq j \leq n$). 
%
Moreover,
%Observe that 
%by imposing the condition that $\sigma(o,p) \neq \emptyset$ for a finite set of pairs $(o,p)$, we are ensuring that each node or edge can have values for a finite number of properties. Thus, as was the case for \tpgs (per Definition~\ref{def:tg}), we have that each \ctpg has a finite representation. Finally, 
observe that two additional conditions are imposed on $\C$, which enforce that a \ctpg conceptually corresponds to a finite sequence of valid conventional property graphs. In particular, as was the case for \tpgs, an edge can only exist at a time when both of the nodes it connects exist, and a property can only take on a value at a time when the corresponding node or edge exists. 
%
%\marcelo{Here add a comment about the running example, explaining how intervals are used.}
%
For instance, assume that $\C = ( \Omega, N, E, \rho, \lambda, \xi, \sigma)$ is a $\ctpg$ corresponding to our running example in Figure \ref{fig:covid}. Then, we have that $\Omega = [1,11]$, $\xi(n_2) = \{[1,9]\}$, $\xi(n_3) = \{[1,7]\}$ and $\xi(e_2) = \{[1,2]\}$, so that $\xi(e_2) \sqsubseteq \xi(n_2)$ and $\xi(e_2) \sqsubseteq \xi(n_3)$. Moreover, for the property risk, we have that $\sigma(n_2,\text{risk}) = \{(\text{low},[1,4]), (\text{high}, [5,9])\}$.

Observe that there is a one-to-one correspondence between TPGs and CTPGs. In particular, a \ctpg $\C = ( \Omega, N, E, \rho, \lambda, \xi, \sigma)$ can be transformed into an equivalent \tpg $\G = ( \Omega', N, E, \rho, \lambda, \xi', \sigma')$ as follows. Assuming that $\Omega = [m,n]$:
\begin{itemize}[leftmargin=4mm]
%\setlength\itemsep{1pt}
\item $\Omega' = \{ i \in \mathbb{N} \mid m \leq i \leq n\}$;

\item for every $o \in (N \cup E)$ and $t \in \Omega'$: $\xi'(o,t) = \true$ if and only if there exists $[a,b] \in \xi(o)$ such that $a \leq t \leq b$;

\item for every $o \in (N \cup E)$, $p \in \Prop$, $t \in \Omega'$ and $v \in \Val$: $\sigma'(o,p,t) = v$ if and only if there exists $(v,[a,b]) \in \sigma(o,p)$ such that $a \leq t \leq b$;
\end{itemize}
The canonical translation of a \ctpg~$\C$, denoted by $\can(\C)$, is defined as the \tpg~$\G$ obtained by using the previous rules. Then, the evaluation of an expression $\pt$ in $\Lthree$ over a \ctpg $\C$ is simply defined by considering its canonical translation, and the definition of the semantics of \Lthree for $\tpgs$:
\begin{eqnarray*}
\semp{\pt}{\C} & = & \semp{\pt}{\can(\C)}.
\end{eqnarray*}
%As the final remark, observe that $(o,t)$ is said to be a temporal object in $\C$ if, and only if, $(o,t)$ is a temporal object in $\can(\C)$.



\iffalse

% \subsection{From property graphs to temporal graphs}

% \pedro{Rewrite}

% \begin{definition}%[\tg]
% \label{def:pg}
% A \pg~is a tuple $\P = (V,E,\rho,\lambda,\sigma)$, where
% %\begin{itemize}%[noitemsep,topsep=3pt,itemindent=\dimexpr\labelwidth+\labelsep\relax,leftmargin=0pt]
% \begin{itemize}
% \item $V$ is a finite set of vertices, $E$ is a finite set of edges,  and $V \cap E = \emptyset$; 

% \item $\rho: E \to (V \times V)$ is a function that maps an edge to its source and destination vertices;

% \item $\lambda: (V \cup E) \to \Lab$ is a function that maps a vertex or an edge to its label;

% \item $\sigma:  (V \cup E) \times \Prop \to \Val$ is a partial function that maps a vertex or an edge, and a property name to a value. Moreover, we assume that there exists a finite number of pairs $(o,p) \in (V \cup E) \times \Prop$ such that $\sigma(o,p)$ is defined.  \qed
% \end{itemize}
% \end{definition}

% Let $\P = (V_1,E_1,\lambda_1,\rho_1,\sigma_1)$ be a \pg~and let $\G = (\Omega, V, E, \lambda, \rho, \xi, \sigma)$ be a \tg. Then $\P$ is said to be the {\em snapshot} of $\G$ at time $t$ if the following conditions are satisfied:
% \begin{itemize}
%     \item $t \in \Omega$;
%     \item $V_1 = \{ v \in V \mid \xi(v,t) = \true\}$;
    
%      \item $E_1 = \{ e \in E \mid \xi(e,t) = \true\}$;
     
%      \item $\rho_1 = \rho|_{E_1}$, that is, $\rho_1$ is the restriction of $\rho$ to the edges in $E_1$;
     
%       \item $\lambda_1 = \lambda|_{V_1 \cup E_1}$, that is, $\lambda_1$ is the restriction of $\lambda$ to the vertices and edges in $V_1 \cup E_1$; and
     
%      \item for every $o \in V_1 \cup E_1$ and $p \in \Prop$,
%      if $\sigma(o,p,t)$ is defined, then $\sigma_1(o,p) = \sigma(o,p,t)$; otherwise, $\sigma_1(o,p)$ is undefined.
% \end{itemize}

% Given a \tg~$\G$, define $\sns(\G) = \{ (\P,t) \mid \P$ is a \pg and $\P$ is the snapshot of $\G$ at time $t \in \Omega \}$. That is,  $\sns(\G)$ is the set of all snapshots of \tg~$\G$, each associated with the time when it occurs.  It is sometimes convenient to treat $\sns(\G)$ as a time-ordered sequence rather than a set. Notice as well that there is a one-to-one correspondence between $\G$ and $\sns(\G)$.

% Observe that in the definition of a \coal \tg $\C$, function $\rho$ and $\lambda$ are used in the same way as for \tgs in Definition~\ref{def:tg}. Function $\xi$ is used to indicate for each vertex or edge $o$, the time intervals where $o$ exists. Given that $\xi(o)$ is a finite family of intervals, we have that $o$ exists only in a finite number of time points in $\N$. Moreover, function $\sigma$ is used to indicate the values of a property $p$ for a vertex or an edge $o$. More precisely, if $\sigma(o,p) = \{(v_1, [a_1, b_1]), \ldots, (v_n, [a_n, b_n])\}$, then the value of property $p$ for $o$ is $v_j$ in every time point in the interval $[a_j, b_j]$ ($1 \leq j \leq n$). 

% Observe that by imposing the condition that $\sigma(o,p) \neq \emptyset$ for a finite number of pairs $(o,p)$, we are ensuring that each vertex or edge can have values for a finite number of properties. Thus, as was the case for \tgs (per Definition~\ref{def:tg}), we have that each \coal \tg has a finite representation. Finally, observe that two additional conditions are imposed on $\C$, which enforce that a \coal \tg~conceptually corresponds to a sequence of valid conventional property graphs. In particular, as was the case for \tg, an edge can only exist at a time when both of the vertices it connects exist, and a property can only take on a value at a time when the corresponding vertex or edge exists. 

% Let $\P = (V_1,E_1,\rho_1,\lambda_1,\sigma_1)$ be a \pg (per Definition~\ref{def:pg})~and $\C = (\Omega, V, E, \rho, \lambda, \xi, \sigma)$ be a \coal \tg ((per Definition~\ref{def:tg1}). Then $\P$ is said to be the \emph{snapshot} of $\C$ at time $t$ if the following conditions are satisfied:
% \begin{itemize}
%     \item $t \in \Omega$
    
%     \item $V_1 = \{ v \in V \mid$ there exists $[a, b] \in \xi(v)$ such that $a \leq t \leq b \}$;
    
%      \item $E_1 = \{ e \in E \mid$ there exists $[a, b] \in \xi(e)$ such that $a \leq t \leq b \}$;
     
%      \item $\rho_1 = \rho|_{E_1}$, that is, $\rho_1$ is the restriction of $\rho$ to the edges in $E_1$;
     
%     \item $\lambda_1 = \lambda|_{V_1 \cup E_1}$, that is, $\lambda_1$ is the restriction of $\lambda$ to the vertices and edges in $V_1 \cup E_1$;
     
%      \item for every $o \in V_1 \cup E_1$ and $p \in \Prop$,
%      if there exists $(v,[a, b]) \in \sigma(o,p)$ such that $a \leq t \leq b$, then $\sigma_1(o,p) = v$; otherwise, $\sigma_1(o,p)$ is not defined.
% \end{itemize}
% %\todo{Pedro: Change notion of equivalence to include time}

% Given a \coal \tg~$\C$, define $\sns(\C) = \{ (\P, t) \mid \P$ is a \pg and $\P$ is the snapshot of $\C$ at time $t\}$. Thus, as was the case for \tg (Definition~\ref{def:tg}), $\sns(\C)$ is the set of all snapshots of a \coal \tg~$\C$, including, for each such snapshot, the time when it occurs.
% Finally, a \coal \tg~$\C$ is said to be equivalent to a \tg~$\G$, denoted by $\C \equiv \G$, if $\sns(\C) = \sns(\G)$.

% \begin{proposition}\label{prop-trans}
% \begin{enumerate}
% \item[(a)] There exists a polynomial-time algorithm that, given a \tg~$\G$, produces a \coal \tg~$\C$ such that $\C \equiv \G$.

% \item[(b)] There exists an exponential-time algorithm that, given a \coal \tg~$\C$, produces a \tg~$\G$ such that $\C \equiv \G$. \qed
% \end{enumerate}
% \end{proposition}

% The canonical translation of a \coal \tg~$\C$, denoted by $\can(\C)$, is defined as the \tg~$\G$ produced by the algorithm mentioned in Proposition \ref{prop-trans} (b). Notice that if a different algorithm is used to produce a \tg~$\G'$ such that $\G'$ is equivalent to $\C$, then $\G'$ represents the same graph as $\can(\C)$ in the sense that $\sns(\G') = \sns(\can(\C)) = \sns(\C)$.

\fi

We conclude this section by defining how a TRPQ is evaluated over a $\ctpg$, and by studying the complexity of evaluation. 

\subsection{Evaluating \Lthree over coalesced temporal property graphs}
%evaluating temporal regular path queries 


In order to understand the complexity of querying a CTPG with an expression in the language $\Lthree$, we introduce the following decision problem parameterized by a query language $\mathcal{L}$. 

\begin{center}
	\framebox{
    	\begin{tabular}{p{1.3cm} p{5.9cm}}
    		\textbf{Problem:} & $\tupleeval(\mathcal{L})$ \\
    		\textbf{Input:} & A \ctpg $\C$, an expression $\pt$ in $\mathcal{L}$ and a pair $(o,t)$, $(o',t')$ of temporal objects in~$\C$ \\
    		\textbf{Output:} & $\true$ if $(o, t, o', t') \in \semp{\pt}{C}$, $\false$ otherwise.
		\end{tabular}
	}
\end{center}

By studying the complexity  of $\tupleeval(\mathcal{L})$ for different fragments $\mathcal{L}$ of $\Lthree$, we can understand how the use of the operators in $\Lthree$ affects the complexity of the evaluation problem and, in particular, which operators are mode difficult to~implement. %Besides, this problem considers the semantics of widely used query languages such as XPath \cite{CD99,M05,GKP05,RDS17}, where the full temporal path is not part of the input.
%
We start our analysis by considering the decision problem associated to the full language.
%, $\Lthree$, which happens to be difficult to evaluate over~\ctpgs:
\begin{theorem}\label{th:LthreeTuplePSPACE}
    $\tupleeval(\Lthree)$ is \pspace-complete.
\end{theorem}
\begin{sloppypar}
Given that $\tupleeval(\Lthree)$ is intractable,
%In the following sections, 
in what follows we look for some natural restrictions of the language for which the evaluation problem is feasible.
\footnote{Proofs of all results presented in this section can be found in the extended version of this paper at \url{https://github.com/marceloarenassaavedra/submission_VLDB2022/blob/master/TRPQ.pdf}.}
%in what following we look for we impose some 
%additional 
%restrictions on $\Lthree$ to understand what are the causes of this high complexity, and to identify classes of queries whose evaluation problem is feasible.
%

%Proof of Theorem \ref{th:LthreeTuplePSPACE}, and of all other results stated in this section, can be found in Appendix \ref{sec-app-proofs}.
\end{sloppypar}

\subsubsection{Removing numerical occurrence indicators}

We start by considering a restriction of our query language in which numerical occurrence indicators are not allowed. Formally, this means that grammar \eqref{grammar:path-expr} is replaced by:
%, we employ the following grammar for path expressions:
\begin{eqnarray}
        \pt & ::= & \test \, \mid \, \axis \, \mid \, (\pt/\pt) \, \mid \, (\pt+\pt)
    \label{grammar:ax-path-expr-no-noi}
\end{eqnarray}
%Notice that every expression in this language is also an expression of \Lthree, so we do not need to redefine its semantics. 
The resulting language is called \Ltwo. The following positive result shows that \Ltwo can be evaluated efficiently over $\ctpgs$, and so is a natural candidate to be implemented in practice:
\begin{theorem}\label{th:LtwoTuplePTIME}
$\tupleeval(\Ltwo)$ can be solved in polynomial time.
\end{theorem}
%\begin{proof}
%See appendix \ref{proof:LtwoTuplePTIME}.
%\end{proof}

\subsubsection{Removing path conditions}

Consider a second restriction of our language in which there are no path conditions. Formally, this means that instead of grammar \eqref{grammar:test}, we use: 
\begin{multline}
        \test \ ::= \  \vd \  \mid \  \ed \  \mid \  \ell \  \mid \  \propt{p}{v} \  \mid \  < \mt \  \mid \  \ex \  \mid \\
        (\test \vee \test) \  \mid \  (\test \wedge \test) \ \mid (\neg \test)
    \label{grammar:test-no-pc}
\end{multline}
%As before, every expression in this language is also an expression of \Lthree, so we do not need to redefine its semantics. 
The resulting language is called \Lonep, for which we get the following result:
%for this restriction:
\begin{theorem}\label{th:LonepSigma2P}
$\tupleeval(\Lonep)$ is \sigmatwop-hard, and it is in $\pspace$.
\end{theorem}
%\begin{proof}
%See appendix \ref{proof:LonepSigma2P}.
%\end{proof}
%
%\subsubsection{No path conditions and numerical occurrence indicators for axis only}
%
A natural question is whether there is a restriction on $\Lonep$ that can reduce the complexity of the evaluation problem but is still expressive enough to represent some useful queries. At this point, a restriction used in the study of XPath comes to the rescue~\cite{M05}. %More precisely, 
%Notice that $\Lonep$ allows numerical occurrence indicators on arbitrary path expressions. A natural question then is whether the complexity of the evaluation problem can be reduced by restricting 
%numerical occurrence 
In what follows, we show that the complexity of the evaluation problem is lower if numerical occurrence indicators
%such indicators to occur 
are only allowed in the axes. 
%In what follows, we give a positive answer to this question. 
%More precisely, consider
%, as before, 
Consider a grammar for tests as in  \eqref{grammar:test-no-pc}, where path conditions are not allowed, and a grammar for path expressions where numerical occurrence indicators are only used in the axes:
%Formally, this means grammar~\eqref{grammar:path-expr} has to be replaced by:
\begin{multline}
    \pt \ ::= \  \test \ \mid \ \axis \ \mid \ \axis[ n, m ] \ \mid \ \axis[n,\_] \ \mid\\
    (\pt/\pt) \ \mid \ (\pt+\pt)
    \label{grammar:ax-path-expr-anoi}
\end{multline}
%Notice that every expression in this language is also an expression of \Lthree, so we do not need to redefine the semantics. 
The resulting language is called \Lonepp, where ANOI refers to numerical occurrence indicators used only in the axes. The following result shows that such a restriction is effective, in the sense that the complexity of the query evaluation problem decreases:
%We get the following result for this restriction:
\begin{theorem}\label{th:LoneppTupleNP}
$\tupleeval(\Lonepp)$ is \np-complete.
\end{theorem}

%\begin{proof}
%See appendix \ref{proof:LoneppTupleNP}.
%\end{proof}

\subsubsection{Allowing numerical occurrence indicators only in the axes}

By the results in the previous sections, $\tupleeval(\Ltwo)$ can be solved in polynomial time, and $\tupleeval(\Lonepp)$ is \np-complete. A natural question 
then is whether the complexity remains the same if these functionalities are combined. Notice that $\tupleeval(\Lthree)$ is $\pspace$-complete, so a positive answer to this question means a significant decrease in the complexity of the query evaluation problem. Unfortunately,  we show that the complexity of the entire language does not decrease by restricting numerical occurrence indicators to occur only in the~axes.
%give a negative answer to this question:
\begin{theorem}\label{th:LthreepTupleNP}
\begin{sloppypar}
$\tupleeval(\Lthreep)$ is \pspace-complete.
\end{sloppypar}
\end{theorem}

%\begin{proof}
%See appendix \ref{proof:LthreepTupleNP}.
%\end{proof}

The results of this section can be considered as a guide for future implementations of $\Lthree$ over coalesced temporal property graphs. The main insight is that the language including path conditions can be efficiently evaluated over such graphs. Besides, a reduction in the complexity for numerical occurrence indicators can be obtained by restricting them to occur only on the axes.

==> proof_t1.tex <==
\begin{figure}[!t]
\caption{Effect of graph size on query execution time, on G1-G6. TEMP}
\label{fig:exp-nodes-size}
\includegraphics[width=\linewidth]{figs/expr/Node-Size-Time-Rel.pdf}
\end{figure}




\subsection{Proof of Theorem \ref{th:LthreeTuplePSPACE}}
\label{proof:LthreeTuplePSPACE}

Consider the following well-known decision problem called True Quantified Boolean Formula ($\tqbf$), which is well known to be \pspace-complete \cite{StockmeyerMeyer1973}:

\begin{center}
	\framebox{
	    \begin{tabular}{p{1.6cm} p{13cm}}
			\textbf{Problem:} & $\tqbf$ \\
		    \textbf{Input:} & A quantified Boolean formula
		    $ \psi = Q_1 x_1 \dots Q_n x_n \, \varphi (x_1, \dots, x_n)$
		    in prenex normal form where $\varphi (x_1, \dots, x_n)$ is a Boolean formula on variables $x_1, \dots, x_n$, and $Q_1, \dots, Q_n$ are quantifiers ($\forall$ or $\exists$). \\
		    \textbf{Output:} & $\true$ if $\psi$ is valid, and $\false$ otherwise.
		\end{tabular}
	}
\end{center}

Without loss of generality, $\varphi$ can be assumed to be in conjunctive normal form. We will show that $\tqbf$ can be reduced to our problem $\tupleeval(\Lthree)$ by proceeding in three steps. Let $\psi = Q_1 x_1 \dots Q_n x_n \, \varphi (x_1, \dots, x_n)$. First, we will show that a predicate $\bit(i,t)$ (defined below) can be written in our language. Then, by using that predicate, we will show that $\varphi$
%(non-quantified) Boolean formula
can be encoded in our language. Finally, we will show that an expression representing  the quantifiers of $\psi$ can be added to the expression encoding $\varphi$, which yields the result.

We start with a $\qbf$ formula $\psi$ as described above to build an input for the problem
$\tupleeval(\Lthree)$. More precisely, the input \ctpg will be $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$ where $\Omega = [0, 2^n-1]$, $N = \lbrace v \rbrace$, $E = \varnothing$, $\rho$ is an empty function, $\lambda(v) = l$, $\xi(v)=\left\lbrace [0, 2^n-1] \right\rbrace$ and $\sigma$ is an empty function. In other words, $\C$ is a \ctpg consisting of only one node existing from time $0$ to time $2^n-1$, with no edges or properties. Moreover, we will build an expression $r$ such that $(v, 0, v, 0) \in \semp{r}{\C}$ if and only if $\psi$ is valid, which concludes the reduction.
%\in \tqbf$, 
The steps to construct $r$ are shown next.
%that we will build with the steps detailed next.

%\hspace{0.5cm}

\bigskip

%\textbf{
{\bf Step 1: Expressing the predicate $\bit$ with an expression in $\Lthree$.}
%
%\hspace{0.5cm}
%
Consider predicate $\bit(i, t)$ that tests whether the $i$-th bit of time $t$ (from right to left when written in its binary representation) is 1. For instance, $\bit(1, 0)$ is false, and $\bit(5, 30)$ is true, since the first bit of $0$ is $0$, whereas $30$ is $11110$ in binary, and its fifth bit is $1$.
Now, consider the following expression:
\begin{eqnarray*}
    r_i &  = & ?\left( \past \left[ 2^i, 2^i \right] \left[ 0, \_ \right] \ / \ \left( < 2^i \wedge \neg < 2^{i-1} \right) \right)
\end{eqnarray*}

Notice that $r_i$ is a test. Thus, for a pair of temporal objects $(o_1, t_1, o_2, t_2)$ %\in \Pt(\C)$ 
to satisfy $r_i$, $(o_1, t_1)$ must be equal to  $(o_2, t_2)$. The expression to satisfy is a path test, so there must be some temporal object $(o_3, t_3)$, such that $(o_1, t_1, o_3, t_3) \in \semp{ \past \left[ 2^i, 2^i \right] \left[ 0, \_ \right] \ /  \left( < 2^i \wedge  \neg < 2^{i-1} \right) }{\C}$.
Since the right part is a test as well, we can split the expression into two parts. Firstly, we must have that $(o_1, t_1, o_3, t_3) \in \semp{ \past \left[ 2^i, 2^i \right] \left[ 0, \_ \right] }{\C}$, which implies that $t_3 = t_1 - k*2^i$ for some integer $k \geq 0$. 
%This means that $t_3$ and $t_1$ are equivalent modulo $2^i$. 
Secondly, we must have that $(o_3, t_3) \models \left( < 2^i \wedge \neg < 2^{i-1} \right)$, which implies that $2^{i-1} \leq t_3 < 2^i$. This means that by writing $t_3$ in its binary form, we get $1$ as its $i$-th bit. Together, these two conditions imply that $t_1$ also has $1$ as its $i$-th bit, when written in its binary form. In consequence, we get that
\begin{align*}
    (o,t, o, t) \in \semp{r_i}{\C} \text{ if and only if } \bit(i, t) \text{ is } \true
\end{align*}
Besides, we trivially get that:
\begin{align*}
    (o,t, o, t) \in \semp{ \neg r_i }{\C} \text{ if and only if } \bit(i, t) \text{ is } \false
\end{align*}
Finally, notice that both $r_i$ and $\neg r_i$ have linear length with respect to $i$, which will be important later.

\bigskip

\textbf{\bf Step 2: Expressing any CNF formula in $\Lthree$.}
Assume that
\begin{eqnarray*}
    \varphi(x_1, \dots, x_n)  &=& \bigwedge_{j=1}^m \bigvee_{k=1}^{m_j} l_{j,k}
\end{eqnarray*}
where for every $j$ and $k$, $l_{j,k}$ is a literal, \textit{i.e.}, either a variable in $\lbrace x_1, \dots, x_n \rbrace$ or its negation. Then, for every $j \in \lbrace 1, \dots, m\rbrace$ and $k \in \lbrace 1, \dots, m_j \rbrace$, we define:
\begin{eqnarray*}
    L_{j,k} &=& \begin{cases}
        r_i & \text{if }  l_{j,k} = x_i \\
        \neg r_i & \text{if  } l_{j,k} = \neg x_i
    \end{cases}
\end{eqnarray*}
    We can use these expressions to build a regular expression that tests the satisfiability of our formula $\varphi(x_1, \dots, x_n)$ by any valuation $\sigma: \left\lbrace x_1, \dots, x_n \right\rbrace \rightarrow \left\lbrace \false, \true \right\rbrace$. To do this, we will use a time value $t \in \left[ 0, 2^n - 1 \right]$ to represent a valuation $\sigma_t$, where $\sigma_t (x_i) = \true$ if and only if the $i$-th bit of $t$ is $1$. We can do so by employing the expressions $L_{i,k}$ on tests along with conjunctions ($\wedge$) and disjunctions ($\vee$), which are also present in $\Lthree$:
\begin{eqnarray*}
    r_{\varphi(x_1, \dots, x_n)} & = & \bigwedge_{j=1}^m \bigvee_{k=1}^{m_j} L_{j, k}
\end{eqnarray*}
Here again, $r_{\varphi(x_1, \dots, x_n)}$ is a test, so if it is satisfied by $(o_1, t_1, o_2, t_2)$, then $(o_1, t_1) = (o_2,t_2)$
%it would be by a pair of repeated temporal objects, say $(o,t, o, t)$. 
Furthermore, we show that, because of how the expressions $L_{j,k}$ are defined, we have:
\begin{align*}
    (o,t, o, t) \in \semp{ r_{\varphi(x_1, \dots, x_n)} }{\C} \text{ if and only if } \sigma_t \left( \varphi(x_1, \dots, x_n) \right) = \true
\end{align*}
%where $\hat{\sigma}_t$ is the natural well-defined extension to any Boolean formula from $\sigma_t$.
%\pedro{Marcelo, please feel free to remove mentions to $\hat{\sigma}$, but maybe first extending the domain to all Boolean formulae from $x_1, \dots, x_n$}
%
To show the previous assertion, first assume that $(o, t, o, t) \in \semp{ r_{\varphi (x_1, \dots, x_n) } }{\C}$. Because of how the expression is defined, for each $j \in \lbrace 1, \dots, m \rbrace$ we must have that $(o, t, o, t) \in \semp{ \bigvee_{k=1}^{m_j} L_{j, k} }{\C}$. Hence, for any arbitrary $j \in \lbrace 1, \dots, m \rbrace$, we immediately get that there must exist $k \in \lbrace 1, \dots, m_j \rbrace$ such that $(o, t, o, t) \in \semp{ L_{j, k} }{\C}$. If $l_{j,k} = x_i$, then we must also have that $(o, t, o, t) \in \semp{r_i}{\C}$, which, as we already showed, is equivalent to having that $\bit(i, t)$ is $\true$, which in turn is equivalent to $\sigma_t(x_i) = \true$. Otherwise, if $l_{j,k} = \neg x_i$, then we must have that $(o, t, o, t) \in \semp{ \neg r_i }{\C}$, which, as we also showed, is equivalent to having that $\bit(i, t)$ is $\false$, which in turn is equivalent to $\sigma_t(x_i) = \false$. In both cases, we get that ${\sigma}_t(l_{j, k}) = \true$, which means that ${\sigma}_t \left( \bigvee_{k=1}^{m_j} l_{j,k} \right) = \true$. Since this holds for an arbitrary value $j$, it holds for the entire conjunction. Hence, ${\sigma}_t \left( \varphi (x_1, \dots, x_n) \right) = \true$.

Now, to show that the inverse is also true, assume that there is some $t \in \Omega$ such that ${\sigma}_t \left( \varphi( x_1, \dots, x_n ) \right) = \true$. By definition, this means that for every $j \in \lbrace 1, \dots, m \rbrace$, ${\sigma}_t \left( \bigvee_{k=1}^{m_j} l_{j, k} \right) = \true$. In turn, this means that for every $j$ there is some $k \in \lbrace 1, \dots, m_j \rbrace$ such that ${\sigma}_t( l_{j, k}) = \true$. As we saw earlier, this condition is equivalent to having that $(o, t, o, t) \in \semp{L_{j,k}}{\C}$, hence, for every $j \in \lbrace 1, \dots, m \rbrace$, we also have that $(o, t, o, t) \in \semp{ \bigvee_{k=1}^{m_j} L_{j,k} }{\C}$. Given that this is true for every $j$, by definition, it is also true for the conjunction of them. Hence, we get that $(o, t, o, t) \in \semp{ r_{\varphi(x_1, \dots, x_n)} }{\C}$. This concludes the proof in Step 2.

\bigskip

\textbf{Observation}: Notice that the previous results already implies $\np$-hardness and $\conp$-hardness for the problem. Since every valuation $\sigma: \lbrace x_1, \dots, x_n \rbrace \rightarrow \lbrace \false, \true \rbrace$ has a corresponding time point $t$ such that $\sigma = \sigma_t$, and a Boolean CNF formula $\varphi (x_1, \dots, x_n)$ on $n$ variables $x_1, \dots, x_n$ is satisfiable if and only if there exists a valuation $\sigma$ such that ${\sigma} \left( \varphi (x_1, \dots, x_n) \right) = \true$, it is also true that $\varphi (x_1, \dots, x_n)$ is satisfiable if and only if $(v, 0, v, 0) \in \semp{ ?(\nxt[0, \_] \ / \ r_{ \varphi (x_1, \dots, x_n) }) }{\C}$ (that is, advance in time to an arbitrary time point $t$ and check the condition that implies that ${\sigma}_t \left( \varphi( x_1, \dots, x_n ) \right) = \true$ for the temporal object $(v, t)$). Similarly, $\varphi(x_1, \dots, x_n) $ is a tautology if and only if $(v, 0, v, 0) \in \semp{\neg ? (\nxt [0, \_] \ / \ \neg r_{\varphi (x_1, \dots, x_n)}) }{\C}$ (there is no path to a time point $t$ such that ${\sigma}_t \left( \varphi( x_1, \dots, x_n ) \right) = \false$, hence there is no valuation that makes $\varphi$ to be $\false$). In what follows, we show $\pspace$-hardness of the problem.

\bigskip

\textbf{Step 3: Expressing satisfiability of quantified Boolean formulae %in prenex normal form 
with an expression in \Lthree.}
Consider a quantified Boolean formula in prenex normal form
\[ Q_1 x_1 \dots Q_n x_n \ \varphi(x_1, \dots, x_n) \]
%with no free variables. 
Since we already have a way to express $\varphi(x_1, \dots, x_n)$, we only need to express the possible valuations (\textit{i.e.}, time points) generated by the sequence of quantifiers $Q_1, \dots, Q_n$.

First, assume $Q_i$ is the existential quantifier ($\exists$). This means that we can either make $x_i$ take valuation $\true$ or $\false$ to satisfy our formula. Considering time points, this is equivalent to have either $1$ or $0$ %respectively 
at the $i$-th bit of the time $t$ at which we are standing. The intuition is that this can easily be expressed by starting at time $0$, and then deciding whether to move into a future time point with the expression $(\nxt [2^{i-1}, 2^{i-1}] + \nxt [0, 0])$ to set the $i$-th bit of the time point. Notice that if there are only expressions of the form $\nxt [2^{i-1}, 2^{i-1}]$, and they are only mentioned once (at least, as prefixes of our test expressions) for each $i$, they will not affect other bits of $t$. Hence, if $s_{i+1}$ represents the part of the subformula $Q_{i+1} x_{i+1} \dots Q_n x_n \ \varphi(x_1, \dots, x_n)$, then the subformula $\exists x_i \ Q_{i+1} x_{i+1} \dots Q_n x_n \ \varphi(x_1, \dots, x_n)$ can be represented by first navigating through time, only affecting the first $i-1$ bits, and then testing that the reached temporal object satisfies the following test:
\begin{eqnarray*} 
s_i & = & ?\left( \left(\nxt [2^{i-1}, 2^{i-1}] + \nxt [0, 0] \right) \ / \ s_{i+1} \right).
\end{eqnarray*}
In turn, if $Q_i$ is the universal quantifier ($\forall$), we will employ the fact that $\forall x \, \psi(x)$ is equivalent to $\neg \exists x \, \neg \psi(x)$ for every formula $\psi(x)$ with free variable $x$. Hence, if $s_{i+1}$ represents the part of the subformula $Q_{i+1} x_{i+1} \dots Q_n x_n \ \varphi(x_1, \dots, x_n)$, then the subformula $\forall x_i \ Q_{i+1} x_{i+1}  \dots Q_n x_n$ $\varphi(x_1, \dots, x_n)$ can be represented by first only navigating through time, only affecting the first $i-1$ bits, and then testing whether the reached temporal object satisfies the following test:
\begin{eqnarray*}
s_i &=& \neg \left( ? \left( (\nxt [2^{i-1}, 2^{i-1}] + \nxt [0, 0]) \ / \ \left(\neg s_{i+1} \right) \right) \right).
\end{eqnarray*}
Finally, define $s_{n+1} = r_{\varphi(x_1, \dots, x_n)}$. We claim that, for $i \in \{ n + 1, n, \dots, 1 \}$ (\textit{i.e.}, $0$ to $n$ quantifiers), if $t < 2^{i - 1}$, then:
\[ (v, t, v, t) \in \semp{s_i}{\C} \ \text{if and only if} \ Q_i x_i \dots Q_n x_n \ \varphi(\sigma_t(x_1), \dots, \sigma_t(x_{i-1}), x_i, \dots, x_n) \ \text{is valid}. \]
In particular, for $n$ quantifiers, \textit{i.e.}, when $i=1$, this result gives us \pspace-hardness for $\tupleeval(\Lthree)$, since we will have that $\psi$ is $\true$ if and only if $(v, 0, v, 0) \in \semp{s_1}{\C}$, where $\C$ and $s_1$ can be constructed in polynomial time in the size of $\psi$. We will prove this claim by induction over the number of quantifiers preceding $\varphi(x_1, \dots, x_n)$.

The base case consists of the formula with no quantified variables, \textit{i.e.}, when $i = n + 1$. We must show that if $t < 2^n$, then $(v, t, v, t) \in \semp{r_{\varphi(x_1, \dots, x_n)}}{\C}$ if and only if $\varphi(\sigma(x_1), \dots, \sigma(x_n))$ is $\true$. Notice that $\varphi(\sigma(x_1), \dots, \sigma(x_n))$ is $\true$
%this membership 
is equivalent to having that ${\sigma}_t(\varphi(x_1, \dots, x_n))$ is $\true$. 
%Since $t$ can take any value below $2^n$, $\sigma_t$ can correspond to any valuation over the $n$ variables, so this is equivalent to the satisfiability of $\varphi(x_1, \dots, x_n)$. 
Hence, by step 2, this is equivalent to having that $(v, t, v, t) \in \semp{r_{\varphi(x_1, \dots, x_n)}}{\C}$.

For the inductive case, assume that the claim holds for $k$ quantifiers, for some $k$ such that $0 \leq k \leq n$. This means that for $i = n - k + 1$, if $t < 2^{i-1}$, then the following condition holds:
\[ (v, t, v, t) \in \semp{s_i}{\C} \ \text{if and only if} \ Q_i x_i \dots Q_n x_n \ \varphi(\sigma_t(x_1), \dots, \sigma_t(x_{i-1}), x_i, \dots, x_n) \ \text{is valid} \]
We then have to prove that the condition holds for $k+1$ quantifiers, \textit{i.e.}, for $i - 1 = n - k$. That is, if $t' < 2^{i-2}$, then we have to show that:
\begin{align}
    \label{eq-equiv-i-1}
(v, t', v, t') \in \semp{s_{i-1}}{\C} \ \text{if and only if} \ Q_{i-1} x_{i-1} \dots Q_n x_n \ \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), x_{i-1}, \dots, x_n) \ \text{is valid}
\end{align}
Let $t' < 2^{i-2}$, and consider the following cases.
\begin{itemize}
    \item If $Q_{i-1} = \exists$, recall that
    \begin{eqnarray*}
        s_{i-1} &=& ? \left( \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ s_{i} \right).
    \end{eqnarray*}
    \begin{sloppypar}
        Notice then that by definition of $s_{i-1}$,
        %a test of the form $(?\pt)$, 
        we have that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$ if and only if there exists $t_1 \in \Omega$ such that $(v, t', v, t_1) \in \semp{ \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ s_i}{\C}$. By definition of $s_i$, 
        %is also a test, so that 
        the previous condition holds if and only if $(v, t', v, t_1) \in \semp{\left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right)}{\C}$ and $(v, t_1, v, t_1) \in \semp{s_i}{\C}$.
    %
        Now, this means that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$ if and only if there exists $t_1 \in \{ t', t' + 2^{i-2} \}$ satisfying that $(v, t_1, v, t_1) \in \semp{s_i}{\C}$.
        
        To prove the direction $(\Rightarrow)$ of \eqref{eq-equiv-i-1} 
        %For the `if' part, 
        assume that $(v,t',v,t') \in \semp{s_{i-1}}{\C}$, which implies that  %suppose that 
        there exists $t_1 \in \{ t', t' + 2^{i-2} \}$ satisfying that $(v, t_1, v, t_1) \in \semp{s_i}{\C}$. Given that $t'$ is an integer with $i-2$ bits, $t_1$ comes from either putting $1$ or $0$ as the $(i-1)$-th bit of $t'$, which means that $t_1 < 2^{i-1}$ must hold. By induction hypothesis, this implies that $Q_i x_i \dots Q_n x_n \varphi(\sigma_{t_1}(x_1), \dots, \sigma_{t_1}(x_{i-1}), x_i, \dots, x_n)$ is valid. Since $t_1$ and $t'$ share the same first $i-2$ bits, we get that $\sigma_{t'}(x_j) = \sigma_{t_1}(x_j)$ for $j \in \{ 1, ..., i-2 \}$. Therefore, we conclude that
        %get by existential introduction that 
        $\exists x_{i-1} Q_i x_i \dots Q_n x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), x_{i-1}, \dots,  x_n)$ is valid.
        
        To prove the direction $(\Leftarrow)$ of \eqref{eq-equiv-i-1} 
        %For the `only if' part, 
        suppose that $\exists x_{i-1} Q_i x_i \dots Q_n x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), x_{i-1}, \dots,  x_n)$ is valid. Then 
        %by existential elimination, 
        we know that $Q_i x_i \dots Q_n x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), b, x_i, \dots,  x_n)$ is valid for some value $b \in \{\true,\false\}$. Define $\mathbbm{1}_b$ as $1$ if $b = \true$, and as $0$ otherwise. Notice then that by taking $t_1 = t' + 2^{i-2} \cdot \mathbbm{1}_b$, we get that $\sigma_{t_1}(x_{i-1}) = b$. Moreover, $\sigma_{t_1}(x_j) = \sigma_{t'}(x_j)$ for every $j \in \{ 1, \dots, i-2 \}$ since $t' < 2^{i-2}$ and $t_1$ shares all its first $i-2$ bits with $t'$. In consequence, this gives us that  $Q_i x_i \dots Q_n x_n \varphi(\sigma_{t_1}(x_1), \dots, \sigma_{t_1}(x_{i-1}), x_i, \dots,  x_n)$ is valid.
        %
        By induction, this means that $(v, t_1, v, t_1) \in \semp{s_i}{\C}$. Since $t_1 = t' + 2^{i-2} \cdot \mathbbm{1}_b$, we have that either $t_1 = t'$ or $t_1 = t' + 2^{i-2}$. In any case, we get that $(v, t', v, t_1) \in \semp{\nxt[2^{i-2}, 2^{i-2}] + \nxt[0, 0] }{\C}$, so we have that $(v, t, v, t_1) \in \semp{(\nxt[2^{i-2}, 2^{i-2}] + \nxt[0, 0] ) \ / \ s_i }{\C}$. By definition of $s_{i-1}$, %expressions of the form $(?\pt)$, this gives us 
        we conclude that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$, which was to be shown.
        %is what we wanted to prove.
    \end{sloppypar}
    
    \item If $Q_{i-1} = \forall$, recall that
    \begin{eqnarray*}
    s_{i-1} &=& \neg ? \left( \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ \left(\neg s_i \right) \right). \end{eqnarray*}
    \begin{sloppypar}
    Now, by definition of $s_{i-1}$,
    %TRPQs of the form $(\neg \test)$, 
    we have that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$ if and only if %it holds that
    \begin{eqnarray*}
    (v, t') & \not\models & ? \left( \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ \left(\neg s_i \right) \right).
    \end{eqnarray*}
    This, in turn, 
    %by definition of TRPQs of the form $(? \pt)$ 
    is equivalent to %having that 
    the fact that there is no time point $t_1 \in \Omega$ such that $(v, t', v, t_1) \in \semp{ \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ \left(\neg s_i \right)}{\C}$.
    %
    Hence, we know that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$ if and only if, for every time point $t_1 \in \Omega$:
    %it holds that
    \[ (v, t', v, t_1) \notin \semp{ \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right) \ / \ \left(\neg s_i \right)}{\C}. \]
    This condition means that each $t_1$ satisfies $(v, t', v, t_1) \notin \semp{ \left(\nxt [2^{i-2}, 2^{i-2}] + \nxt [0, 0] \right)}{\C}$ or $(v, t_1) \not\models \left(\neg s_i \right)$. This, in turn, is equivalent to saying that if $t_1 \in \{ t', t' + 2^{i-2} \}$ then $(v, t_1) \not\models \left(\neg s_i \right)$, \textit{i.e.}, $(v, t_1) \models s_i $.
    % 
    As a consequence, $(v, t', v, t') \in \semp{s_{i-1}}{\C}$ if and only if $(v, t') \models s_i$ and $(v, t' + 2^{i-2}) \models s_i$, which is equivalent to having that $(v, t', v, t') \in \semp{s_i}{\C}$ and $(v, t' + 2^{i-2}, v, t' + 2^{i-2}) \in \semp{s_i}{\C}$.
    
    
    To prove the direction ($\Rightarrow$) of \eqref{eq-equiv-i-1} suppose that $(v, t', v, t') \in \semp{s_{i-1}}{\C}$, so we also have that $(v, t', v, t') \in \semp{s_i}{\C}$ and $(v, t' + 2^{i-2}, v, t' + 2^{i-2}) \in \semp{s_i}{\C}$. Notice then that $t' < 2^{i-2}$, so $t'$ and $t' + 2^{i-2}$ are both smaller than $2^{i-1}$. By induction hypothesis, we get then that both quantified Boolean formulae $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-1}), x_i, \dots, x_n)$ and $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t' + 2^{i-2}}(x_1), \dots, \sigma_{t' + 2^{i-1}}(x_{i-1}), x_i, \dots, x_n)$ are valid.
    %
    Furthermore, since $t'$ is smaller than $2^{i-2}$, $\sigma_{t'}(x_{i-1}) = \false$, and since $t' + 2^{i-2}$ only differs from $t'$ in its $(i-1)$-th bit, which is $1$, we get that $\sigma_{t' + 2^{i-2}}(x_{i-1}) = \true$ and, for every $j \in \{ 1, \dots, {i-2} \}$, it holds that $\sigma_{t'}(x_j) = \sigma_{t' + 2^{i-2}}(x_j)$. Hence, both quantified Boolean formulae $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), \false, x_i, \dots, x_n)$ and $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), \true, x_i, \dots, x_n)$ are valid. Therefore, %By universal generalization, 
    we conclude that the quantified Boolean formula $\forall x_{i-1} Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), x_{i-1}, x_i, \dots, x_n)$ is valid.
    
    To show the direction ($\Leftarrow$) of \eqref{eq-equiv-i-1} suppose that $\forall x_{i-1} Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), x_{i-1}, x_i, \dots, x_n)$ is valid. Then
    %By universal elimination, 
    we get that both quantified Boolean formulae $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), \false, x_i, \dots, x_n)$ and $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-2}), \true, x_i, \dots, x_n)$ are valid.
    %
    As before, since $t'$ is smaller than $2^{i-2}$, $\sigma_{t'}(x_{i-1}) = \false$, and since $t' + 2^{i-2}$ only differs from $t'$ in its $(i-1)$-th bit, which is 1, we get that $\sigma_{t' + 2^{i-2}}(x_{i-1}) = \true$ and for every $j \in \{ 1, \dots, {i-2} \}$, it holds that $\sigma_{t'}(x_j) = \sigma_{t' + 2^{i-2}}(x_j)$. This allows us to conclude that both $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t'}(x_1), \dots, \sigma_{t'}(x_{i-1}), x_i, \dots, x_n)$ and $Q_i x_i \dots Q_{n} x_n \varphi(\sigma_{t' + 2^{i-2}}(x_1), \dots, \sigma_{t' + 2^{i-1}}(x_{i-1}), x_i, \dots, x_n)$ are valid.
    %
    Finally, by induction hypothesis, this implies that $(v, t', v, t') \in \semp{s_i}{\C}$ and $(v, t' + 2^{i-2}, v, t' + 2^{i-2}) \in \semp{s_i}{\C}$, which, as shown before, holds if and only if $(v, t', v, t') \in \semp{s_{i-1}}{\C}$, which concludes the proof for this case.
    \end{sloppypar}
\end{itemize}
As we mentioned, all this together implies that $\tupleeval(\Lthree)$ is \pspace-hard, since \ctpg $\C$, expression $s_1$ and tuple $(v, 0, v, 0)$ can be constructed in polynomial time in the size of $\psi$, and the problem of determining whether $\psi$ is valid 
%a True Quantified Boolean Formula 
can be reduced to the problem of verifying whether $(v, 0, v, 0) \in \semp{s_1}{\C}$.

Thus, it only remains to show that $\tupleeval(\Lthree)$ is in \pspace. To do this, we will provide an algorithm in \pspace that, given a \ctpg \C, an expression $r$ in \Lthree, and a tuple $(o, t, o', t') \in \Pt(\C)$, computes whether $(o,t, o',t') \in \semp{r}{\C}$. More precisely, Algorithm $\textsc{TupleEvalSolve}\left(\C, r, (o_1, t_1, o_2, t_2)\right)$ is defined as follows.

\LinesNumbered

\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{A \ctpg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, an expression $r$ in $\Lthree$ and a pair of temporal objects $(o_1, t_1, o_2, t_2) \in \Pt(\C)$}
    \Output{$\true$ if and only if $(o_1,t_1, o_2,t_2) \in \semp{r}{\C}$}
    \uIf{$r$ is a test}{
        \uIf{$(o_1, t_1) \neq (o_2, t_2)$}{
            \Return \false
        }
        \uIf{$r = \vd$}{
            \Return $(o_1 \in N)$
        }
        \uElseIf{$r = \ed$}{
            \Return $(o_1 \in E)$
        }
        \uElseIf{$r = \ell$ for some \ $\ell \in \Lab$}{
            \Return $\lambda(o_1) = \ell$
        }
        \uElseIf{$r = \propt{p}{v}$ for some $p\in \Prop$ \ \text{and} $v\in \Val$}{
            \ForEach{valued interval $(v', I) \in \sigma(o_1, p)$}{
                \uIf{$t_1 \in I$}{
                    \Return $(v' = v)$
                }
            }
        }
        \uElseIf{$r = \, < \mt$ with $\mt \in \Omega$}{
            \Return $(t_1 < \mt)$
        }
        \uElseIf{$r = \ex$}{
            \ForEach{interval $I \in \xi(o_1)$}{
                \uIf{$t_1 \in I$}{
                    \Return \true
                }
            }
        }
        \uElseIf{$r = (?r')$}{
            \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                \uIf{$\textsc{TupleEvalSolve}\left(\C, r', (o_1, t_1, o', t') \right)$}{
                    \Return \true
                }
            }
        }
        \uElseIf{$r = (\test_1 \vee \test_2)$}{
            \Return $\textsc{TupleEvalSolve}\left(\C, \test_1, (o_1, t_1, o_1, t_1) \right) \ \textbf{or} \ \textsc{TupleEvalSolve}\left(\C, \test_2, (o_1, t_1, o_1, t_1) \right)$
        }
        \uElseIf{$r = (\test_1 \wedge \test_2)$}{
            \Return $\textsc{TupleEvalSolve}\left(\C, \test_1, (o_1, t_1, o_1, t_1) \right) \ \textbf{and} \ \textsc{TupleEvalSolve}\left(\C, \test_2, (o_1, t_1, o_1, t_1) \right)$
        }
        \uElseIf{$r  = \left( \neg r' \right)$}{
            \Return $\textbf{not} \ \textsc{TupleEvalSolve}\left(\C, r', (o_1, t_1, o_1, t_1) \right)$
        }
    }
    \uElseIf{$r = \nxt$}{
        \Return $o_1 = o_2 \ \textbf{and} \ t_2 = t_1 + 1$
    }
    \uElseIf{$r = \prv$}{
        \Return $o_1 = o_2 \ \textbf{and} \ t_2 = t_1 - 1$
    }
    \uElseIf{$r = \fw$}{
        \Return $t_1 = t_2 \ \textbf{and} \ \left(
            \left( o_1 \in E \ \textbf{and} \ o_2 = \tgt(o_1) \right)
            \ \textbf{or} \
            \left( o_2 \in E \ \textbf{and} \ o_1 = \src(o_2) \right)
        \right)$
    }
    \uElseIf{$r = \bw$}{
        \Return $t_1 = t_2 \ \textbf{and} \ \left(
            \left( o_1 \in E \ \textbf{and} \ o_2 = \src(o_1) \right)
            \ \textbf{or} \
            \left( o_2 \in E \ \textbf{and} \ o_1 = \tgt(o_2) \right)
        \right)$
    }
    \uElseIf{$r  = \left(r_1 + r_2 \right)$}{
        \Return $\textsc{TupleEvalSolve}\left(\C, r_1, (o_1, t_1, o_2, t_2) \right) \ \textbf{or} \ \textsc{TupleEvalSolve}\left(\C, r_2, (o_1, t_1, o_2, t_2) \right)$
    }
    \uElseIf{$r = \left(r_1 \ / \ r_2 \right)$}{
        \ForEach{$(o',t') \in (N \cup E) \times \Omega$}{
            \uIf{$\textsc{TupleEvalSolve}\left(\C, r_1, (o_1, t_1, o', t') \right) \textbf{and} \ \textsc{TupleEvalSolve}\left(\C, r_2, (o', t', o_2, t_2) \right)$}{
                \Return $\true$
            }
        }
    }
    \caption{$\textsc{TupleEvalSolve}\left(\C, r, (o_1, t_1, o_2, t_2)\right)$ (part I)}
\end{algorithm}

\begin{algorithm}
    %\ContinuedFloat
    \SetAlgoLined
    \setcounter{AlgoLine}{43}
    \uElseIf{$r = r' \left[ n, m \right]$}{
        \uIf{$m = n$}{
            \uIf{$n = 0$}{
                \Return $(o_1, t_1) = (o_2, t_2)$
            }
            \uElseIf{$n = 1$}{
                \Return $\textsc{TupleEvalSolve} \left( \C, r', (o_1, t_1, o_2, t_2) \right)$
            }
            $l \gets \lfloor n/2 \rfloor$ \\
            \uIf{$m $ is even}{
                \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                    \uIf{$\textsc{TupleEvalSolve} \left( \C, r'[ l, l], (o_1, t_1, o', t') \right)
                    \textbf{and} \ 
                    \textsc{TupleEvalSolve} \left( \C, r'[ l, l], (o', t', o_2, t_2) \right)$}{
                        \Return $\true$
                    }
                }
            }
            \uElseIf{$m$ is odd}{
                \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                    \ForEach{$(o'', t'') \in (N \cup E) \times \Omega$}{
                        \uIf{$($\\
                        $\qquad \textsc{TupleEvalSolve}\left( \C, r'[ l, l ], (o_1, t_1, o', t') \right)
                        \textbf{and} $ \\
                        $\qquad \textsc{TupleEvalSolve}\left( \C, r', (o', t', o'', t'') \right)
                        \textbf{and} $ \\
                        $\qquad \textsc{TupleEvalSolve}\left( \C, r'[ l, l ], (o', t', o_2, t_2) \right)$ \\
                        $)$}{
                            \Return $\true$
                        }
                    }
                }
            }
        }
        \uElseIf{$n = 0$}{
            \uIf{$m = 1$}{
                $\Return (o_1, t_1) = (o_2, t_2) \ \ \textbf{or} \ \ \textsc{TupleEvalSolve} \left( \C, r', (o_1, t_1, o_2, t_2) \right)$
            }
            $l \gets \lfloor m/2 \rfloor$ \\
            \uIf{$m$ is even}{
                \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                    \uIf{$\textsc{TupleEvalSolve} \left( \C, r'[ 0, l], (o_1, t_1, o', t') \right)
                    \textbf{and} \ 
                    \textsc{TupleEvalSolve} \left( \C, r'[ 0, l], (o', t', o_2, t_2) \right)$}{
                        \Return $\true$
                    }
                }
            }
            \uElseIf{$m$ is odd}{
                \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                    \ForEach{$(o'', t'') \in (N \cup E) \times \Omega$}{
                        \uIf{
                            $($ \\
                            $\qquad \textsc{TupleEvalSolve}\left( \C, r'[ 0, l ], (o_1, t_1, o', t') \right) \ \textbf{and} $ \\
                            $\qquad \textsc{TupleEvalSolve}\left( \C, r'[ 0, 1 ], (o', t', o'', t'') \right) \ \textbf{and}$ \\
                            $\qquad \textsc{TupleEvalSolve}\left( \C, r'[ 0, l ], (o', t', o_2, t_2) \right)$ \\
                            $)$
                        }{
                            \Return $\true$
                        }
                    }
                }
            }
        }
        \uElse{
            \ForEach{$(o', t') \in (N \cup E) \times \Omega$}{
                \uIf{$\textsc{TupleEvalSolve}\left( \C, r'[ n, n ], (o_1, t_1, o', t') \right) \textbf{and} \  \textsc{TupleEvalSolve}\left( \C, r'[ 0, m-n ], (o', t', o_2, t_2) \right)$}{
                    \Return $\true$
                }
            }
        }
    }
    \uElseIf{$r = r' \left[ n, \_ \right]$}{
        $m \gets n + (\left| \Omega \right| \cdot \left| N \cup E \right|)^2$ \\
        \Return $\textsc{TupleEvalSolve}\left(\C, r'[n, m], (o_1, t_1, o_2, t_2) \right)$
    }
    \Return \false
    \caption{$\textsc{TupleEvalSolve}\left(\C, r, (o_1, t_1, o_2, t_2)\right)$ (part II)}
\end{algorithm}

Next we show that
%We will prove that  is in \pspace by showing that, 
for every \ctpg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, expression $r$ in $\Lthree$ and tuple $(o_1, t_1, o_2, t_2) \in \Pt(\C)$, it holds that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $\textsc{TupleEvalSolve} \left(\C, r, (o_1, t_1, o_2, t_2) \right)$ returns $\true$. Besides, we will prove that 
$\textsc{TupleEvalSolve}$ works in polynomial space in the size of the input.
%while using only polynomial space.

Notice firstly that the algorithm is recursive, and that the depth of the recursion is polynomial, since at every step on which the algorithm is called, the size of the path expression strictly decreases. There is one exception, that happens when $r$ is of the form $\pt[n, \_]$. Notice that here this expression is treated as if it was $\pt[n, m]$, where $m = n + \left| \Omega \right| \cdot \left| N \cup E \right|$ (a term with polynomial size with respect to the input). Thus, the whole expression $r$ can be thought as an equivalent expression $r'$ where all terms of the form $\pt[n, \_]$ are replaced with similar ones, in a manner that makes the whole input remain polynomial to the original. Although it might seem that $\pt[n, m]$ could reach an exponential number of recursive calls, notice that this expression is always parsed as two expressions, $\pt[n, n]$ and $\pt[0, m-n]$, and then each of those is solved in a way similar to that of exponentiation by squaring, which allows to always get rid of the numerical occurrence indicator $[n, m]$ after at most $O(\log m)$ recursive calls, a number that is polynomial in the size of the input. Hence the recursion tree has polynomial height.

Secondly, assume that conjunctions ($\wedge$) and disjunctions ($\vee$) are computed from left to right, \textit{i.e.}, $A(x) \wedge A(y)$ first computes $A(x)$ and then computes $A(y)$. Hence, at the most, we will need to have in memory as many calls to the algorithm as the recursion tree height. This number is polynomial, and since every non-recursive step is either a non-deterministic guess or clearly in polynomial time in the size of the input, we get that the whole algorithm gives an answer in \pspace.

Now, let  $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$ be a \ctpg, let $r$ be an expression in $\Lthree$ and let $(o_1, t_1, o_2, t_2) \in \Pt(\C)$ be a tuple concatenating two temporal objects. First suppose that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. We will show, by induction on the recursion level of the recursion tree, that there exists an execution of algorithm $\textsc{TupleEvalSolve} \left( \C, r, (o_1, t_1, o_2, t_2) \right) $ that returns $\true$. Notice that the base case is given for those cases where there is no recursion.
%
The base test cases, \textit{i.e.}, when $r$ is equal to either $\vd$, $\ed$, $\ell$, $\propt{p}{v}$, $<\mt$, or $\ex$, are easily checked, since all the algorithm does is checking their definitions over the temporal object $(o_1, t_1)$ after checking that it is equal to the temporal object $(o_2, t_2)$. Notice that for property-value checking and existence checking, the default value is $\false$, returned at the end of the algorithm.
%
The base navigation operators $\nxt$, $\prv$, $\fw$ and $\bw$ are also easily checked by their definitions. For time navigation, we check that the objects are the same and that their associated times are consecutive, whereas for spatial navigation, we check that the times are equal, and that the respective objects are consecutive, by looking at the functions $\tgt$ and $\src$, as defined by the operators.

As for the recursive cases, assume that the property holds up to recursion level $n$ and we want to prove that it holds at recursion level $n-1$ (one level higher in the recursion tree).
%
Firstly, a path expression matching any of the regular expressions $(\test \wedge \test)$, $(\test \vee \test)$ or $(\neg \test)$ can also be checked quite straightforwardly by definition, and since the flow is deterministic, we will omit further formal proofs.
%
Secondly, if the path expression $r$ is of the form $(?r')$, then we know that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only $(o_1, t_1) = (o_2, t_2)$ and there exists a temporal object $(o', t') \in \Pt(\C)$ such that $(o_1, t_1, o', t') \in \semp{r'}{\C}$. In such case, the algorithm iterates one by one over the possible temporal objects to find one that satisfies the condition. If such temporal object exists, the call to $\textsc{TupleEvalSolve}$ returns $\true$, since we then know that the tuple $(o_1, t_1, o', t')$ satisfies $r'$ if and only if there exist an execution of the call that returns $\true$. Conversely, if no such temporal object exists, all recursive calls to $\textsc{TupleEvalSolve}$ will return $\false$ by induction hypothesis. In this case, the algorithm will finish the loop without returning and it will then reach the last line (in part II), returning $\false$.

As for regular path expressions $r$ of the form $(r_1 + r_2)$ where $r_1$ and $r_2$ are also regular path expressions, we know that by definition $\semp{(r_1 + r_2)}{\C} = \semp{r_1}{\C} \cup \semp{r_2}{\C}$. Hence, $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r_1}{\C}$ or $(o_1, t_1, o_2, t_2) \in \semp{r_2}{\C}$. By induction hypothesis, this means that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if either $\textsc{TupleEvalSolve}(\C, r_1, (o_1, t_1, o_2, t_2))$ returns $\true$ or $\textsc{TupleEvalSolve}(\C, r_2, (o_1, t_1, o_2, t_2))$ returns $\true$. As the algorithm returns the disjunction of this two results, we get that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $\textsc{TupleEvalSolve}(\C, r, (o_1, t_1, o_2, t_2))$ returns $\true$

For regular path expressions $r$ of the form $(r_1 \ / \ r_2)$ where $r_1$ and $r_2$ are also TRPQs, we know that if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$, then there must exist a temporal object $(o',t') \in \Pt(\C)$ such that $(o_1, t_1, o', t') \in \semp{r_1}{\C}$ and $(o', t', o_2, t_2) \in \semp{r_2}{\C}$. Thus, by iterating over all temporal object $(o',t')$, when we reach that exact temporal object, both $\textsc{TupleEvalSolve}(\C, r_1, (o_1, t_1, o', t'))$ and $\textsc{TupleEvalSolve}(\C, r_2, (o', t', o_2, t_2))$ will be $\true$, so the algorithm will return $\true \ \textbf{and} \ \true = \true$. On the other hand, if $(o_1, t_1, o_2, t_2) \notin \semp{r}{\C}$, then no matter what temporal object $(o', t')$ is being considered, we will either have that $(o_1, t_1, o', t') \notin \semp{r_1}{\C}$ or $(o', t', o_2, t_2) \notin \semp{r_2}{\C}$. By induction hypothesis, this means that, for every execution, either the first call will be $\false$ or the second will, so the condition that makes the algorithm return $\true$ will not be met. Hence, the last line is reached and the algorithm returns $\false$.

For expressions $r$ matching regular expressions with numerical occurrence indicators of the form $r'[n, m]$, recall that, by definition, $\semp{r'[n, m]}{\C} = \bigcup_{k=n}^m \semp{r'^k}{\C}$. This implies that $(o_1, t_1, o_2, t_2) \in \semp{r'[n, m]}{\C}$ if and only if there exists an integer $k \in [n, m]$ such that $(o_1, t_1, o_2, t_2) \in \semp{r'^k}{\C}$. We split this case into three cases.

\begin{enumerate}
    \item When $n = m$, then $(o_1, t_1, o_2, t_2) \in \semp{r'[n, m]}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r'^n}{\C}$. Recall that the concatenation operator is associative, and that $\semp{r'^n}{\C} = \semp{r' \ / \ r'^{n-1}}{\C} = \semp{r' \ / \ \dots \ / \ r'}{\C}$ ($n$ repetitions). Hence, if we define $l = \lfloor n/2 \rfloor$, then if $n$ is even, $\semp{r'^n}{\C} = \semp{(r'^l \ / \ r'^l)}{\C}$, whereas if $n$ is odd, $\semp{r'^n}{\C} = \semp{(r'^l \ / \ r' \ / \ r'^l)}{\C}$.

    In the first case then, by the definition of concatenation, $(o_1, t_1, o_2, t_2) \in \semp{(r'^l \ / \ r'^l)}{\C}$ if and only if there exists a temporal object $(o', t')$ such that $(o_1, t_1, o', t') \in \semp{r'^l}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'^l}{\C}$. By induction hypothesis this is equivalent to having that there exists a temporal object $(o', t')$ such that both $\textsc{TupleEvalSolve}(\C, r'[l, l], (o_1, t_1, o', t'))$ and $\textsc{TupleEvalSolve}(\C, r'[l, l], (o', t', o_2, t_2))$ return $\true$, since $\semp{r'^l}{\C} = \semp{r'[l, l]}{\C}$. Since the algorithm iterates over all possible temporal objects to check this condition, if such temporal object exists, it will return $\true$, if it does not, then it will reach the last line and return $\false$.

    The second case is similar, except that now we need two temporal objects as there are two concatenations, which means that $(o_1, t_1, o_2, t_2) \in \semp{(r'^l \ / \ r' \ / \ r'^l)}{\C}$ if and only if there exist two temporal objects $(o', t')$ and $(o'', t'')$ such that $(o_1, t_1, o', t') \in \semp{r'^l}{\C}$, $(o', t', o'', t'') \in \semp{r'}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r'^l}{\C}$. By induction hypothesis, and recalling again that $\semp{r'^l}{\C} = \semp{r'[l, l]}{\C}$, that means that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exist two temporal objects $(o', t')$ and $(o'', t'')$ such that the calls $\textsc{TupleEvalSolve}(\C, r'[l, l], (o_1, t_1, o', t'))$, $\textsc{TupleEvalSolve}(\C, r', (o', t', o'', t''))$ and $\textsc{TupleEvalSolve}(\C, r'[l, l], (o'', t'', o_2, t_2))$ return $\true$. Again, since the algorithm iterates over all possible pairs of temporal objects $(o', t')$ and $(o'', t'')$ to check this condition, if such temporal objects exist, it will return $\true$, if it does not, then it will reach the last line and return $\false$.
    
    Since this recursion must stop at some point, the base case $n = 1$ is included, in which case $r$ is $r'[1, 1]$, which is equivalent to $r'$, since in such case we know that $(o_1, o_2, t_1, t_2) \in \semp{r}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r'}{C}$. By hypothesis induction, this happens if and only if $\textsc{TupleEvalSolve}(\C, r', (o_1, t_1, o_2, t_2))$ returns $\true$, which is why the algorithm returns that result.
    
    Finally, the recursion works for $n \geq 2$. The case when $n = 1$ is covered as a base case, so it only remains to look for the case when $n = 0$. For such case, recall that $r'^0 = (\exists \vee \neg \exists)$, \textit{i.e.}, a test that is a tautology. Hence, $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $(o_1, t_1) = (o_2, t_2)$, which is what the algorithm tests.
    
    \item When $n = 0$, the base case will be slightly different. We can assume that $n \neq m$ since the case where $n = m$ was already covered. Hence, the base case only needs to consider the value $m = 1$. In this case, we have that $\semp{r}{\C} = \semp{r'[0, 1]}{\C} = \semp{r'^0}{\C} \cup \semp{r'^1}{\C}$. As we already discussed, checking whether $(o_1, t_1, o_2, t_2) \in \semp{r'^0}{\C}$ comes down to checking whether $(o_1, t_1) = (o_2, t_2)$, and also $\semp{r'^1}{\C} = \semp{r'}{\C}$. By induction, we know that $(o_1, t_1, o_2, t_2) \in \semp{r'}{\C}$ if and only if $\textsc{TupleEvalSolve}(\C, r', (o_1, t_1, o_2, t_2))$ returns $\true$. Since the algorithm returns $\true$ if either of these conditions hold, this case is correctly covered.
    
    As for the recursive case, it is very similar to the previous one. If we define again $l = \lfloor m/2 \rfloor$, we can notice that, if $m$ is even, then $\semp{r'[0, m]}{\C} = \semp{(r'[0, l] \ / \ r'[0,l])}{\C}$, whereas if $m$ is odd, then $\semp{r'[0, m]}{\C} = \semp{(r'[0, l] \ / \ r' \ / \ r'[0,l])}{\C}$.
    
    To show the part when $m$ is even, notice that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r'^i}{\C}$ for some $i \in [0, m]$. For every $i \in [0, m]$ there exist two integers, $j_i := \lfloor i/2 \rfloor$ and $k_i := \lceil i/2 \rceil$, both in the interval $[0, l]$, that satisfy that $j_i + k_i = i$. Since the concatenation operator is associative, this means that $\semp{r'_i}{\C} = \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$, which in turn implies that $\semp{r}{\C} = \bigcup_{i=0}^m \semp{r'_i}{\C} = \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$.
    
    Then, by definition of the concatenation operator, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$ if and only if there exists a temporal object $(o', t')$ such that $(o_1, t_1, o', t') \in \semp{r'^{j_i}}{\C}$ and $(o', t', o_2, t_2) \in \semp{r^{k_i}}{\C}$.
    
    Since both $j_i$ and $k_i$ are bounded by $l$, $\semp{r'^{j_i}}{\C} \subseteq \semp{\bigcup_{i=0}^l r'^i}{\C}$, and $\semp{r'^{k_i}}{\C} \subseteq \semp{\bigcup_{i=0}^l r'^i}{\C}$, so any tuple $(o, t, o', t')$ in $\semp{r'^{k_i}}{\C}$ or $\semp{r'^{j_i}}{\C}$ will also be in $\semp{\bigcup_{i=0}^l r'^i}{\C} = \semp{r'[0, l]}{\C}$. Hence, $(o_1, t_1, o', t') \in \semp{r'^{j_i}}{\C}$ implies that $(o_1, t_1, o', t') \in \semp{r'[0, l]}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'^{k_i}}{\C}$ implies that $(o', t', o_2, t_2) \in \semp{r'[0, l]}{\C}$. It can then be inferred that having that $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$ can only hold if there exists a temporal object $(o', t')$ satisfying that $(o_1, t_1, o', t') \in \semp{r'^[0, l]}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'[0, l]}{\C}$. As a result, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$ implicates that $(o_1, t_1, o_2, t_2) \in \semp{(r'[0, l] \ / \ r'[0, l])}{\C}$. In consequence, we get that $\bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C} \subseteq \semp{(r'[0, l] \ / \ r'[0, l])}{\C}$.
    
    For the inverse inclusion, notice that if $(o_1, t_1, o_2, t_2) \in \semp{(r'[0, l] \ / \ r'[0, l])}{\C}$, then there must exist a temporal object $(o', t')$ and two integers $j$ and $k$ in $[0, l]$ such that $(o_1, t_1, o', t') \in \semp{r'^j}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'^k}{\C}$, which implies that $(o_1, t_1, o_2, t_2) \in \semp{(r'^j \ / \ r'^k)}{\C}$. Again, since concatenation is associative, $\semp{(r'^i \ / \ r'^j)}{\C} = \semp{r'^{i+j}}{\C}$, and because $i + j$ is at most $n$, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^n \semp{r'^i}{\C}$, \textit{i.e.}, $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. As a result, we get that $\semp{(r'[0, l] \ / \ r'[0, l])}{\C} \subseteq \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$.
    
    Combining these two inclusions with the equality $\semp{r}{\C} = \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$, we get that $\semp{r}{\C} = \semp{(r'[0, l] \ / \ r'[0, l])}{\C}$.
    
    To show the part where $n$ is odd, notice that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists an integer $i \in [0, m]$ such that $(o_1, t_1, o_2, t_2) \in \semp{r'^i}{\C}$. Notice then that $i$ can be written as the sum of three integers, $k_i := \lfloor i/2 \rfloor$ ($\in [0, l]$), $j_i =: \lfloor i/2 \rfloor$ ($\in [0, l]$) and $s_i := (i mod 2)$ ($\in [0, 1]$). Since the concatenation operator is associative, this means that $\semp{r'_i}{\C} = \semp{(r'^{j_i} \ / \ r'^{s_i} \ / \ r'^{k_i})}{\C}$, which in turn implies that $\semp{r}{\C} = \bigcup_{i=0}^m \semp{r'_i}{\C} = \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{s_i} \ / \ r'^{k_i})}{\C}$.
    
    Then, by definition of the concatenation operator, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{s_1}\ / \ r'^{k_i})}{\C}$ if and only if there exist two temporal objects $(o', t')$ and $(o'', t'')$ such that $(o_1, t_1, o', t') \in \semp{r'^{j_i}}{\C}$, $(o', t', o'', t'') \in \semp{r'^{s_i}}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r'^{k_i}}{\C}$.
    
    Since both $j_i$ and $k_i$ are bounded by $l$, $\semp{r'^{j_i}}{\C} \subseteq \semp{\bigcup_{i=0}^l r'^i}{\C}$, and $\semp{r'^{k_i}}{\C} \subseteq \semp{\bigcup_{i=0}^l r'^i}{\C}$, so any tuple $(o, t, o', t')$ in $\semp{r'^{k_i}}{\C}$ or $\semp{r'^{j_i}}{\C}$ will also be in $\semp{\bigcup_{i=0}^l r'^i}{\C} = \semp{r'[0, l]}{\C}$. Similarly, any tuple in $\semp{r'^{s_1}}{\C}$ will also be in $\semp{r'[0,1]}{\C}$. Hence, $(o_1, t_1, o', t') \in \semp{r'^{j_i}}{\C}$ implies that $(o_1, t_1, o', t') \in \semp{r'[0, l]}{\C}$, $(o', t', o'', t'') \in \semp{r'^{s_i}}{\C}$ implies that $(o', t', o'', t'') \in \semp{r'[0, 1]}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r^{k_i}}{\C}$ implies that $(o'', t'', o_2, t_2) \in \semp{r[0, l]}{\C}$. It can then be inferred that having that $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^m \semp{(r'^{j_i} \ / \ r'^{s_i} \ / \ r'^{k_i})}{\C}$ can only hold if there exist two temporal objects $(o', t')$ and $(o'', t'')$ satisfying that $(o_1, t_1, o', t') \in \semp{r'^[0, l]}{\C}$, $(o', t', o'', t'') \in \semp{r'[0, 1]}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r[0, l]}{\C}$. As a result, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$ implicates that $(o_1, t_1, o_2, t_2) \in \semp{(r'[0, l] \ / \ r'[0, 1] \ / \ r'[0, l])}{\C}$. In consequence, we get that $\bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C} \subseteq \semp{(r'[0, l] \ / \ r'[0, 1] \ / \ r'[0, l])}{\C}$.
    
    For the inverse inclusion, notice that if $(o_1, t_1, o_2, t_2) \in \semp{(r'[0, l] \ / \ r'[0, 1] \ / \ r'[0, l])}{\C}$, then there must exist two temporal objects $(o', t')$ and $(o'', t'')$, and three integers $j \in [0, l]$, $s \in [0, 1]$ and $k \in [0, l]$ such that $(o_1, t_1, o', t') \in \semp{r'^j}{\C}$, $(o'', t'') \in \semp{r'^s}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r'^k}{\C}$, which implies that $(o_1, t_1, o_2, t_2) \in \semp{(r'^j \ / \ r'^s \ / \ r'^k)}{\C}$. Again, since concatenation is associative, $\semp{(r'^i \ / \ r'^s \ / \ r'^j)}{\C} = \semp{r'^{i+ s + j}}{\C}$, and because $i + s + j$ is at most $n$, $(o_1, t_1, o_2, t_2) \in \bigcup_{i=0}^n \semp{r'^i}{\C}$, \textit{i.e.}, $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. As a result, we get that $\semp{(r'[0, l] \ / \ r'[0, 1] \ / \ r'[0, l])}{\C} \subseteq \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{k_i})}{\C}$.

\begin{sloppypar}    
    As before, combining these two inclusions with the equality $\semp{r}{\C} = \bigcup_{i=0}^n \semp{(r'^{j_i} \ / \ r'^{l_i} \ / \ r'^{k_i})}{\C}$, we get that $\semp{r}{\C} = \semp{(r'[0, l] \ / \ r'[0, 1] \ / \ r'[0, l])}{\C}$.
    With these two results in mind then, \textit{i.e.}, that $\semp{r'[0, m]}{\C} = \semp{(r'[0, l] \ / \ r'[0,l])}{\C}$ when $m$ is even, whereas if $m$ is odd, then $\semp{r'[0, m]}{\C} = \semp{(r'[0, l] \ / \ r' \ / \ r'[0,l])}{\C}$, we know that $(o_1, t_1, o_2, t_2) \in \semp{r'[0, m]}{\C}$ if and only if (i) $m$ is even and there exists a temporal object $(o', t')$ such that $(o_1, t_1, o', t') \in \semp{r'[0,l]}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'[0, l]}{\C}$, or (ii) $m$ is odd and there exist two temporal objects $(o', t')$ and $(o'', t'')$ such that $(o_1, t_1, o', t') \in \semp{r'[0, l]}{\C}$, $(o', t', o'', t'') \in \semp{r'[0, 1]}{\C}$ and $(o'', t'', o_2, t_2) \in \semp{r'[0, l]}{\C}$.
    
    By induction, (i) holds if and only if there exists a temporal object $(o', t')$ such that both $\textsc{TupleEvalSolve}(\C, r'[0, l], (o_1, t_1, o', t'))$ and $\textsc{TupleEvalSolve}(\C, r'[0, l], (o', t', o_2, t_2))$ return $\true$. Since the algorithm iterates over all temporal objects $(o', t')$ for this case, and then checks that both those conditions are met to return $\true$, it will return $\true$ if $(i)$ holds, and it will reach the last line and return $\false$ if no such pair existed.
    
    Also by induction, (ii) holds if and only if there exist two temporal objects $(o', t')$ and $(o'', t'')$ such that the three calls $\textsc{TupleEvalSolve}(\C, r'[0, l], (o_1, t_1, o', t'))$, $\textsc{TupleEvalSolve}(\C, r'[0, l], (o', t', o'', t''))$ and $\textsc{TupleEvalSolve}(\C, r'[0, l], (o'', t'', o_2, t_2))$ return $\true$. 
    Here again, since the algorithm iterates over all pairs of temporal objects $(o', t')$ and $(o'', t'')$ and sees if these three conditions are met to return $\true$, it will return $\true$ if (ii) holds, and it will reach the last line and return $\false$ otherwise.
    
    Hence, when $n = 0$, the algorithm also returns $\true$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$
    
    \item When $m \neq n$ and $n \neq 0$, then $(o_1, t_1, o_2, t_2) \semp{r'[n, m]}{\C}$ if and only if there exists $i \in [n, m]$ such that $(o_1, t_1, o_2, t_2) \semp{r'^i}{\C}$. In this case, $i = n + d$ for some $d \in [0, m-n]$, and since the concatenation operator is associative, $(o_1, t_1, o_2, t_2) \semp{r'^i}{\C}$ if and only if there exists $(o', t')$ such that $(o_1, t_1, o', t') \in \semp{r'^n}{\C}$ and $(o', t', o_2, t_2) \in \semp{r'^d}{\C}$. 
    By induction, and since $\semp{r'^n}{\C} = \semp{r'[n, n]}{\C}$, $(o_1, t_1, o', t') \in \semp{r'^n}{\C}$ if and only if $\textsc{TupleEvalSolve}(\C, r'[n, n], (o_1, t_1, o', t'))$. Similarly, $(o', t', o_2, t_2) \in \semp{r'^d}{\C}$ for some $d \in [0, m-n]$ if and only if $(o', t', o_2, t_2) \in \semp{r'[0, m-n]}{\C}$, which by induction holds if and only if $\textsc{TupleEvalSolve}(\C, r'[0, m-n], (o', t', o_2, t_2))$.

    Together, this means that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists a temporal object $(o', t')$ such that $\textsc{TupleEvalSolve}(\C, r'[n, n], (o_1, t_1, o', t')$ and $\textsc{TupleEvalSolve}(\C, r'[0, m-n], (o', t', o_2, t_2))$. Since the algorithm iterates over all temporal objects $(o', t')$ and checks if these conditions are met to return $\true$, it will return $\true$ if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ and it will reach the last line and return $\false$ otherwise.
    \end{sloppypar}
\end{enumerate}
Finally, for an expression $r$ matching a regular expressions with numerical occurrence indicators of the form $r'[n, \_]$, recall that we showed in Section \ref{sec-navl-compl} that $\semp{r'[n, \_]}{\C} = \semp{r'[n, m}{\C}$, where the expression $m := n + (|\Omega| + |V \cup E|)^2$ is polynomial in the size of the original input.
%
By induction, $(o_1, t_1, o_2, t_2) \in \semp{r'[n, m]}{\C}$ if and only if $\textsc{TupleEvalSolve}(\C, r'[n, m], (o_1, t_1, o_2, t_2))$ returns $\true$, which is what the algorithm returns for this case.
Altogether, we proved that $\textsc{TupleEvalSolve}$ works in polynomial space, and that $\textsc{TupleEvalSolve}(\C, r, (o_1, t_1, o_2, t_2))$ returns $\true$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. 
%This completes the proof needed to show that $\tupleeval(\Lthree)$ is in \pspace. This, along, with the previous result, implies \pspace-completeness, so the theorem follows.
This concludes the proof of the theorem.

==> proof_t2.tex <==
\subsection{Proof of Theorem \ref{th:LtwoTuplePTIME}}
\label{proof:LtwoTuplePTIME}

First of all notice that basic tests such as $\vd$, $\ed$, $\ell$, $\propt{p}{v}$, $<\mt$ and $\ex$ can be checked in $O(1)$, so in absence of numerical occurrence indicators, checking a test is equivalent to checking the satisfaction of a Boolean formula on a given valuation, which can be done efficiently in time $O(n)$, where $n$ is the size of the formula. We will assume in the following then that we have a linear-time function $\textsc{CheckTestNoPC}(\C, (o, t), \test)$ that takes as input a \ctpg $\C$, a temporal object $(o, t)$ in $\C$ and a test expression $\test$ in $\Ltwo$, and returns $\true$ if $(o, t) \models \test$ in $\C$, and $\false$ otherwise.

To show that $\tupleeval(\Ltwo)$ is in \ptime, we present a polynomial-time procedure in Algorithm \ref{algo:TupleEvalSolveOnlyPC}, called $\textsc{TupleEvalSolveOnlyPC}$, that, given a \ctpg $\C$, a tuple representing a pair of temporal objects $(o_1, t_1, o_2, t_2)$ and an expression $r$ in $\Ltwo$, checks whether $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. In what follows, we show that
Algorithm \ref{algo:TupleEvalSolveOnlyPC} works in polynomial time.
%We also claim that this is done in polynomial time. To show this, have a look at algorithm \ref{algo:TupleEvalSolveOnlyPC} below.

\LinesNumbered

\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Initialization}{Initialization}
    \Input{\ A \ctpg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, an expression $r$ in $\Ltwo$ and a pair of temporal objects $\left( o_1, t_1, o_2, t_2 \right) \in \Pt(\C)$}
    \Output{\ $\true$ if $\left( o_1, t_1, o_2, t_2 \right) \in \semp{r}{\C}$, and $\false$ otherwise}
    \Initialization{
        \ A global variable $H$ initially empty, storing a hash table with the currently computed values for $\textsc{TupleEvalSolveOnlyPC}$. \\
    }
    \uIf{$\left( o_1, t_1, o_2, t_2, r \right)$ is a key in hash table $H$}{
        \Return $H[\left( o_1, t_1, o_2, t_2, r \right)]$
    }
    \uIf{$r = \nxt$}{
        $A \gets \left(
            o_1 = o_2 \ \textbf{and} \ t_2 = t_1 + 1
        \right)$
    }
    \uElseIf{$r = \prv$}{
        $A \gets \left(
            o_1 = o_2 \ \textbf{and} \ t_2 = t_1 - 1
        \right)$
    }
    \uElseIf{$r = \fw$}{
        $A \gets \left(
            t_1 = t_2 \ \textbf{and} \ \left(
                \left( o_1 \in E \ \textbf{and} \ o_2 = \tgt\left( o_1 \right) \right)
                \ \textbf{or} \
                \left( o_2 \in E \ \textbf{and} \ o_1 = \src\left( o_2 \right) \right)
            \right)
        \right)$
    }
    \uElseIf{$r = \bw$}{
        $A \gets \left(
            t_1 = t_2 \ \textbf{and} \ \left(
                (o_1 \in E \ \textbf{and} \ o_2 = \src(o_1))
                \ \textbf{or} \
                (o_2 \in E \ \textbf{and} \ o_1 = \tgt(o_2))
            \right)
        \right)$
    }
    \uElseIf{$r$ is a test}{
        $A \gets \left( 
            ( o_1, t_1) = ( o_2, t_2)
            \ \textbf{and} \
            \textsc{CheckTestNoPC}( \C, ( o_1, t_1), r)
        \right)$
    }
    \uElseIf{$r = (r_1 + r_2)$}{
        %$(r_1 + r_2) \gets r$ \\
        $A \gets \textsc{TupleEvalSolveOnlyPC}(
            \C, ( o_1, t_1, o_2, t_2), r_1
        )$ \\
        \uIf {$\textbf{not} A$}{
            $A \gets \textsc{TupleEvalSolveOnlyPC}(
                \C, ( o_1, t_1, o_2, t_2), r_2
            )$
        }
    }
    \uElseIf{$r = (r_1 \ / \ r_2)$}{
        %$(r_1 \ / \ r_2) \gets r$ \\
        $A \gets \false$ \\
        $l_1 \gets \| r_1 \|$ \\
        $l_2 \gets \| r_2 \|$ \\
        \ForEach{$(o, t) \in (N \cup E) \times \{ t \in \Omega \ \mid \ \left( |t - t_1| \leq l_1 \ \wedge \ |t - t_2| \leq l_2 \right) \}$}{
            \uIf{\textsc{TupleEvalSolveOnlyPC}$(\C, (o_1, t_1, o, t), r_1)$}{
                \uIf{\textsc{TupleEvalSolveOnlyPC}$(\C, (o, t, o_2, t_2), r_2)$} {
                    $A \gets \true$ \\
                    \textbf{break}
                }
            }
        }
    }
    Store the value $A$ for $\textsc{TupleEvalSolveOnlyPC}(\C, (o_1, t_1, o_2, t_2), r)$ in the hash table $H$ with key $(o_1, t_1, o_2, t_2, r)$ \\
    \Return $A$
    \caption{$\textsc{TupleEvalSolveOnlyPC}(\C, (o_1, t_1, o_2, t_2), r)$}
    \label{algo:TupleEvalSolveOnlyPC}
\end{algorithm}

Notice first that we do not directly return the result. Instead, we first look at a hashing table that stores previously stored results, and only if this was not previously computed, we compute the result for the input, and store it in the table before returning the value. We employ this to avoid an exponential number of calls when recursively calling the algorithm.
%
This is possible since, in absence of numerical occurrence indicators, navigation is done at most one step at a time. Thus, if $(o_2,t_2)$ is a temporal object reached from $(o_1, t_1)$ using an expression $r$, then $|t_1 - t_2|$ is at most 
%will have a time that differs in a number that is bounded by 
the number of 
%equal to 
%at most as many  
symbols $\nxt$ and $\prv$ occurring in $r$. Hence, if $\|r\|$ is the length of expression $r$, then there are at most $O(\| r \| \cdot | N \cup E |)$ temporal objects that we will need to consider for this call, which means, at most $O(\| r \|^2 \cdot | N \cup E |^2)$ tuples representing pairs of temporal objects. Hence, given that there are at most $\| r \|$ sub-expressions of $r$ that can be reached
%added to the fact that 
in the tree decomposition of $r$, we need to store at most $O(\| r \|^3 \cdot | N \cup E |^2)$ different results for $\textsc{TupleEvalSolveOnlyPC}$.

The rest of the algorithm is quite straightforward, and it considers the case when the %for whenever the 
result has not been precomputed. If $r$ is a temporal navigation operator, then by the definitions of $\nxt$ and $\prv$, a single temporal object can be reached, $(o_1, t_1+1)$ or $(o_1, t_1-1)$, respectively, so we check that $(o_2, t_2)$ is equal to that respective temporal object. This can be easily done in $O(1)$.
%
If $r$ is a spatial navigation operator, then we have to look at the mapping from edges to source and destination nodes, $\rho$, to determine the set of objects that can be reached. If $o$ is an edge, and we move forward, we look for its destination node, if we move backward, for its source node. If $o$ is a node, and we move forward, we are looking for the edges that have $o$ as their source, and if we move backward, then we look for those who have $o$ as their destination. The whole process can be done in time $O(\| \rho \|)$, which is $O(\| \C \|)$.
%
When $r$ is testing a condition, we just call the previously mentioned algorithm $\textsc{CheckTestNoPC}$ to check whether $(o, t) \models r$ in $\C$. This last base case can be done in time $O(\|r\|)$.

When $r$ is of the form $(r_1 + r_2)$, where $r_1$ and $r_2$ are expressions in $\Ltwo$, we have that $(o_1, t_1, o_2, t_2) \in \semp{(r_1 + r_2)}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r_1}{\C}$ or $(o_1, t_1, o_2, t_2)  \in \semp{r_2}{\C}$, so if suffices that the call to $\textsc{TupleEvalSolveOnlyPC}$ with any of inputs $r_1$ or $r_2$ returns $\true$, and this can be easily checked by the algorithm.
%
The last case is when $r$ is of the form $(r_1 \ / \ r_2)$ where $r_1$ and $r_2$ are expressions in $\Ltwo$, where we have that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if there exists a temporal object $(o, t)$ such that $(o_1, t_1, o, t) \in \semp{r_1}{\C}$ and $(o, t, o_2, t_2) \in \semp{r_2}{\C}$. We know that in absence of numerical occurrence indicators, $t$ will be at distance at most $\|r_1\|$ from $t_1$ and at most $\|r_2\|$ from $t_2$, since one can move only as many times as there are $\nxt$ and $\prv$ symbols in the respective formulas, so this gives us a polynomial-size set from which we can extract candidates to satisfy this condition.

Finally, notice that at every call to $\textsc{TupleEvalSolveOnlyPC}(\C, (o_1, t_1, o_2, t_2), r)$, we either already have computed the value for the key $(o_1, t_1, o_2, t_2, r)$, in which case we can give an answer immediately, or we are computing a new value to store in the hash table $H$, which has size bounded by $O(\| r \|^3 \cdot | N \cup E |^2)$. In any case, since the most expensive step performs at most $O(| N \cup E | \cdot \| r \|)$ recursive calls, we will be getting an answer in time $O(\| r \|^4 \cdot | N \cup E |^3)$, which is polynomial in the size of the input.


==> proof_t3.tex <==
\subsection{Proof of Theorem \ref{th:LonepSigma2P}}
\label{proof:LonepSigma2P}

Consider the following decision problem called Generalized Subset Sum (\gsss) which is known to be \sigmatwop-complete \cite{Berman2001}:

\begin{center}
	\framebox{
	    \begin{tabular}{p{1.6cm} p{11cm}}
			\textbf{Problem:} & $\gsss$ \\
		    \textbf{Input:} & 
		    Natural numbers vectors $u$ and $w$ of dimensions $\dim(u)$ and $\dim(w)$, respectively, 
		    %in $\bigcup_{k \geq 1}\mathbb{N}^k$, 
		    and a positive integer $S \in \mathbb{N}$ \\
		    \textbf{Output:} & $\true$ if there exists $x \in \{0, 1\}^{\dim(u)}$ such that, for all $y \in \{0, 1\}^{\dim(w)}$, it holds that $x\cdot u + y \cdot w \neq S$, and $\false$ otherwise.
		\end{tabular}
	}
\end{center}
In this problem, $a \cdot b$ represents the inner product between vectors $a$ and $b$.
Given vectors $u = (u_1, \dots, u_n) \in \mathbb{N}^n$ and $w = (w_1, \dots, w_m) \in \mathbb{N}^m$, and the integer $S \in \mathbb{N}$, the goal is to provide a polynomial-time algorithm that returns 
%many-one reduction to 
a \ctpg $\C$, a tuple $(o_1, t_1, o_2, t_2)$, and an expression $r$ in $\Lonep$ such that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $\exists x \in \{0, 1\}^n \ \forall y \in \{ 0, 1 \}^m \ x \cdot u + y \cdot w \neq S$.

Let $M = 2 \cdot \left(\sum_{i=1}^n u_i + \sum_{j=1}^m w_j \right)$, which can be easily computed in polynomial time from $u$ and $w$. Then $\C$ will be the \ctpg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$ where $\Omega = [0, 2 \cdot M]$, $N = \lbrace v \rbrace$, $E = \varnothing$, $\rho$ is an empty function, $\lambda(v) = l$, $\xi(v)=\left\lbrace [0, 2 \cdot M] \right\rbrace$ and $\sigma$ is an empty function. In other words, $\C$ is a \ctpg consisting of only one node existing from time $0$ to time $2 \cdot M$, with no edges or properties. The tuple $(o_1, t_1, o_2, t_2)$ in our reduction will be given by $(v, M, v, 2 \cdot M)$.
%
As for the expression $r$, it will be defined recursively as follows. First define an expression for each component $u_i$ of $u$ that will represent whether $u_i \cdot x_i$ will be chosen to be $u_i$ or $0$:
\begin{eqnarray*} 
r_{u_i} &=& \nxt [u_i, u_i] [0, 1].
\end{eqnarray*}
The idea is that the time $t$ of the temporal object that is being reached will store the sum given by $x \cdot u + y \cdot w$, plus $M$ to avoid having negative numbers on the time dimension when testing that the result 
%the condition of having something 
is different from $S$ (this will be explained in more detail later). 
%
Define then an expression for $u$, representing the sum accumulated by the $\exists x \in \{0, 1\}^n$ part of the problem:
\begin{eqnarray*}
r_u &=& r_{u_1} \ / \ \dots \ / \ r_{u_n}.
\end{eqnarray*}
We will now use a recursive construction to represent the sum accumulated by the $\forall y \in \{ 0, 1 \}^m$ part of the problem. First define condition $r_{t \neq S + M}$, that represents that the accumulated sum is not $S$:
\begin{eqnarray*}
    r_{t\neq S + M}  & = & (< S + M \vee \neg < S + M + 1)
\end{eqnarray*}
By taking $r_0 := r_{t \neq S + M}$, now recursively define $r_{j + 1}$ from $r_j$, for $j \in \{ 0, \dots, m - 1 \}$, as follows:
\begin{eqnarray*}
r_{j + 1} &=& \left( \nxt [w_{j + 1}, w_{j + 1}] \ / \ r_j \ / \ \prv [2 \cdot w_{j + 1}, 2 \cdot w_{j + 1}] \right) \left[ 2, 2 \right] \ / \ \nxt [ 2 \cdot w_{j + 1}, 2 \cdot w_{j + 1} ]
\end{eqnarray*}
The formula $r_w = r_m$ will allow to iterate over all the accumulated sums implied by the $\forall y \in \{ 0, 1 \}^m$ part of the problem. Finally, $r$ is defined as follows:
\begin{eqnarray*}
r &=& r_u \ / \ r_w \ / \ \nxt[0, \_] \ / \ (\neg < 2 \cdot M )
\end{eqnarray*}
We now prove that $(v, M, v, 2 \cdot M) \in \semp{r}{\C}$ if and only if $\exists x \in \{0, 1\}^n \ \forall y \in \{ 0, 1 \}^m \ x \cdot u + y \cdot w \neq S$.

Assume that both $t$ and $t'$ are in $\Omega$. By induction on the definition of numerical occurrence indicators, it is easy to see that $(v, t, v, t') \in \semp{\nxt[k, k]}{\C}$ if and only if $t' = t + k$. Hence, by definition of $r_{u_i}$, we have that $(v, t, v, t') \in \semp{r_{u_i}}{\C}$ if and only if $t' = t$ (0 occurrences) or $t' = t + u_i$ (1 occurrence), or what is equivalent, if there exists $x_i \in \{ 0, 1 \}$ such that $t' = t + x_i \cdot u_i$. 
%
In fact, it can be proved by induction that $(v, t, v, t') \in \semp{r_u}{\C}$ if and only if $\exists x \in \{ 0, 1 \}^n$ such that $t' = t + x \cdot u$. We will demonstrate something stronger, which is that $(v, t, v, t') \in \semp{r_{u_1} \ / \ \dots \ / r_{u_i}}{\C}$ if and only if there exists $(x_1, \dots, x_i) \in \{ 0, 1 \}^i$ such that $t' = t + \sum_{k=1}^i x_i \cdot u_i$.

Our base case will be checking the property for $r_{u_1}$, which, by the same exact reasoning as above, satisfies that $(v, t, v, t') \in \semp{r_{u_1}}{\C}$ if and only if there exists $x_1 \in \{ 0, 1 \}$ such that $t' = t + x_1 \cdot u_1$.
%
Suppose now that $(v, t, v, t') \in \semp{r_{u_1} \ / \ \dots \ / r_{u_i}}{\C}$ if and only if there exists $(x_1, \dots, x_i) \in \{ 0, 1 \}^i$ such that $t' = t + \sum_{k=1}^i x_i \cdot u_i$. We also know by the previous reasoning that $(v, t', v, t'') \in \semp{r_{u_{i+1}}}{\C}$ if and only if there exists $x_{i+1} \in \{ 0, 1 \}$ such that $t'' = t' + x_{i+1} \cdot u_{i+1}$. Hence, by definition of $(r_1 / r_2)$, we get that $(v, t, v, t'') \in \semp{r_{u_1} \ / \ \dots \ / r_{u_{i+1}}}{\C}$ if and only if there exists $(v, t')$ such that there exists $(x_1, \dots, x_i) \in \{ 0, 1 \}^i$ such that $t' = t + \sum_{k=1}^i x_i \cdot u_i$ and there exists $x_{i+1} \in \{ 0, 1 \}$ such that $t'' = t' + x_{i+1} \cdot u_{i+1}$, \textit{i.e.}, if and only if there exists $(x_1, \dots, x_{i+1}) \in \{ 0, 1 \}^{i+1}$ such that $t'' = t + \sum_{k=1}^{i+1} x_i \cdot u_i$. This yields the result.

%In particular, this means that $(v, M, v', t') \in \semp{r_u}{\C}$ if and only if $\exists x \in \{ 0, 1 \}^n$ such that $t' = M + x \cdot u$.

Moreover, by definition of $\semp{(r_1 / r_2)}{\C}$, we get that $(v, M, v, 2 \cdot M) \in \semp{r}{\C}$ if and only if there exists $x \in \{ 0, 1 \}^n$ such that:
\[(v, M + x \cdot u, v, 2 \cdot M) \in \semp{r_v \ / \ \nxt[0, \_] \ / \ (\neg < 2 \cdot M )}{\C}\]
Notice also that the right part of this formula is built in the following way:  $(\neg < 2 \cdot M)$ is a test that is only satisfied by $(v, 2 \cdot M, v, 2 \cdot M)$, whereas $\nxt[0, \_]$ is satisfied by any tuple $(v, t, v, t')$ such that $t \leq t'$. Hence, $(v, t, v', t') \in \semp{ \nxt[0, \_] \ / \ (\neg < 2 \cdot M )}{\C}$ if and only if $t$ is any time point in $\Omega$ and $t' = 2 \cdot M$.
%
Thus, all we need to prove now is that there exists some time point $t$ such that $(v, M + x \cdot u, v, t) \in \semp{r_v}{\C}$ if and only if $\forall y \in \{0, 1\}^m \ x \cdot u + y \cdot w \neq S $.

%We will show that time point $t$ to equal exactly $M + x \cdot u$. To prove this, 
First, we show  %notice that it can be proved 
by induction that if $(v, t, v, t') \in \semp{r_j}{\C}$, then $t = t'$. The base case is trivial, since $r_0$ is a test.
For the inductive case, 
%whereas the inductive case is shown by the following sequence:
%\begin{enumerate}
    %\item 
assume that if $(v, t, v, t') \in \semp{r_j}{\C}$, then $t' = t$.
    %\item 
    For conciseness, define $a := w_{j+1}$. In the case of $j + 1$, we know that if $(v, t_1, v, t_2) \in \semp{\nxt[a,a] \ / \ r_j \ / \ \prv[2a, 2a]}{\C}$, then there exist time points $t_3$ and $t_4$ such that $(v, t_1, v, t_3) \in \semp{\nxt[a, a]}{\C}$, $(v, t_3, v, t_4) \in \semp{r_j}{\C}$ and $(v, t_4, v, t_2) \in \semp{\prv[2a, 2a]}{\C}$. Notice then that these conditions only hold respectively if $t_3 = t_1 + a$, by definition of operator $\nxt$ and numerical occurrence indicators, $t_3 = t_4$ by induction hypothesis and $t_2 = t_4 - 2a$. Thus, $t_2 = t4 - 2a = t_3 - 2a = t_1 - a$.
    %\item 
    %We repeat that expression twice because of NOI $[2, 2]$, so 
    It is clear that if $(v, t_1, v, t_5) \in \semp{(\nxt[a,a] \ / \ r_k \ / \ \prv[2a, 2a])[2, 2]}{\C}$, then $t_5 = t_1 - 2a$.
    %\item 
    Finally, if $(v, t_5, v, t') \in \semp{\nxt[2a, 2a]}{\C}$, then $t' = t_5 + 2a$, so by definition of $\semp{(r_1/ r_2)}{\C}$, we conclude  that if $(v, t, v, t') \in \semp{r_{j+1}}{\C}$, then $t' = t$.
%\end{enumerate}

Given the conclusion in the previous paragraph,
%Now, 
all we need to prove now is that $(v, M + x \cdot u, v, M + x \cdot u) \in \semp{r_v}{\C}$ if and only if $\forall y \in \{0, 1\}^m \ x \cdot u + y \cdot w \neq S $.
%
In fact, we will prove by induction a stronger condition:
%that is, that:
\[
\text{for every } k \in \{0, \dots, m\}, \text{it holds that }
\forall y \in \{0, 1\}^k \ t + \sum_{j=1}^k y_j \cdot w_j \neq S \text{ if and only if }
(v, M +  t, v, M + t) \in \semp{r_k}{\C} \]
The case when $t = x \cdot u$ and $k = m$ yields Theorem \ref{th:LonepSigma2P} as a result.
%
In the base case $k = 0$, we need to prove that %where this case, we want to prove that 
$t \neq S$ if and only if $(v, M + t, v, M + t) \in \semp{r_0}{\C}$. Recall that $r_0 = r_{t \neq S + M}$. It can be easily checked that $(v, t) \models r_0$ if and only if $t \neq S + M$. Also, $r_0$ is a test, so $(v, t, v, t') \in \semp{r_0}{\C}$ if and only if $t = t'$ and $t \neq S + M$. Hence, we have that $(v, M + t, v, M + t) \in \semp{r_0}{\C}$ if and only if $ M +  t =  M + t$ (which is trivially satisfied) and $M +  t \neq M + S$,
\textit{i.e.}, if and only if $t \neq S$.
For the inductive case, assume that for $k \in \{0, \dots, m\}$, it holds that:
%it holds that 
\[\forall y \in \{0, 1\}^k \ t + \sum_{j=1}^k y_j \cdot w_j \neq S \text{ if and only if }
(v, M + t, v, M + t) \in \semp{r_k}{\C}.\]
Then we have to prove that:
\[\forall y \in \{0, 1\}^{k + 1} \ t + \sum_{j=1}^{k+1} y_j \cdot w_j \neq S 
\text{ if and only if }
(v, M + t, v, M + t) \in \semp{r_{k+1}}{\C} \]
To prove this, define again $a := w_{k+1}$ for conciseness. Recall that $r_{k + 1} = ((\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a])[2,2] / \nxt[2a, 2a])$. Notice then that $(v, M + t, v, t') \in \semp{\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a]}{\C}$ if and only if there exist time points $t_1$ and $t_2$ such that $(v, M + t, v, t_1) \in \semp{\nxt[a, a]}{\C}$, $(v, t_1, v, t_2) \in \semp{r_k}{\C}$ and $(v, t_2, v, t') \in \semp{\prv[2a, 2a]}{\C}$.
%
The first condition is equivalent to having that $t_1 = M + t + a$. The second condition implies that $t_1 = t_2$, given what we proved in the previous paragraphs. Hence, given that $(v, M + t + a, v, M + t + a) \in \semp{r_k}{\C}$, we conclude by induction hypothesis that 
%By induction, the second condition holds if and only if 
$\forall y \in \{ 0, 1 \}^k \ t + a + \sum_{j=1}^k y_j \cdot w_j \neq S$. 
%By what we just proved, it also implies that $t_2 = t_1$. 
The third condition is equivalent to having that $t' = t_2 - 2a$. Altogether, this means that $(v, M + t, v, t') \in \semp{\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a]}{\C}$ if and only if $t' = M + t - a$ and $\forall y \in \{ 0, 1 \}^k$, it holds that $t + a + \sum_{j=1}^k y_j \cdot w_j \neq S$.
%
Now, this means that $(v, M + t, v, t') \in \semp{(\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a])[2, 2]}{\C}$ if there exists a time point $t''$ such that $t'' = M + t - a$, $t' = M + (t-a) - a = M + t - 2a$, $\forall y \in \{ 0, 1 \}^k$, it holds that $t + a + \sum_{j=1}^k y_j \cdot w_j \neq S$, and $\forall y \in \{ 0, 1 \}^k$, it holds that $(t - a) + a + \sum_{j=1}^k y_j \cdot w_j \neq S$.
Therefore,
%Hence, altogether this means that 
$(v, M + t, v, t') \in \semp{(\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a])[2, 2]}{\C}$ if and only if $t' = M + t - 2a$ and for every $y \in \{ 0, 1 \}^{k+1}$, it holds that $t + \sum_{j=1}^{k+1} y_j \cdot w_j \neq S$.
Given that
for $t_1, t_2 \in \Omega$, it holds that $(v, t_1, v, t_2) \in \semp{\nxt[2a, 2a]}{\C}$ if and only if $t_2 = t_1 + 2a$, we conclude that $(v, M + t, v, t') \in \semp{(\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a])[2, 2] \ / \ \nxt [2a, 2a]}{\C}$ if and only if $t' = M + t$ and $\forall y \in \{ 0, 1 \}^{k+1} \ t + \sum_{j=1}^{k+1} y_j \cdot w_j \neq S$.
%
Finally, this gives us the result we are trying to prove, that is, $(v, M + t, v, M + t) \in \semp{(\nxt[a, a] \ / \ r_k \ / \ \prv[2a, 2a])[2, 2] \ / \ \nxt [2a, 2a]}{\C}$ if and only if $\forall y \in \{ 0, 1 \}^{k+1} \ t + \sum_{j=1}^{k+1} y_j \cdot w_j \neq S$.
%which, as said before, implies our theorem.

To conclude the proof of the theorem, notice that $r$ can be constructed in polynomial time with respect to the sizes of $u$, $v$ and $S$, so the entire reduction can be computed in  polynomial time.
%, and that the results hold only when the time points are within $\Omega$, which is ensured by the choice of $M$. This concludes the proof. \qed

==> proof_t4.tex <==
\subsection{Proof of Theorem \ref{th:LoneppTupleNP}}
\label{proof:LoneppTupleNP}

To show \np-hardness, consider the following decision problem called Subset Sum (\sss), which is known to be \np-complete \cite{SubsetSum1990}:

\begin{center}
	\framebox{
	    \begin{tabular}{p{1.6cm} p{10cm}}
			\textbf{Problem:} & $\sss$ \\
		    \textbf{Input:} & A finite set of integers $A \subsetneq \mathbb{N}$, and a positive integer $S \in \mathbb{N}$ \\
		    \textbf{Output:} & $\true$ if there exists a subset $A' \subseteq A$ of $A$ such that $\sum_{a \in A'} a = S$.
		\end{tabular}
	}
\end{center}
Given a set $A \subsetneq \mathbb{N}$, and an integer $S \in \mathbb{N}$, the goal is to provide a polynomial-time algorithm that returns a \ctpg $\C$, a tuple $(o_1, t_1, o_2, t_2)$, and an expression $r$ in $\Lonepp$ such that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists $A' \subseteq A$ such that $\sum_{a \in A'} a = S$.
More specifically,
%In this occasion, 
$\C$ will be the \ctpg $\left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$ where $\Omega = [0, S]$, $N = \lbrace v \rbrace$, $E = \varnothing$, $\rho$ is an empty function, $\lambda(v) = l$, $\xi(v)=\left\lbrace [0, S] \right\rbrace$ and $\sigma$ is an empty function. In other words, $\C$ is a \ctpg consisting of only one node existing from time $0$ to time $S$, with no edges or properties. The tuple $(o_1, t_1, o_2, t_2)$ in our reduction will be given by $(v, 0, v, S)$. Moreover, assuming that $A = \{ a_1, \dots, a_n \}$, expression $r$ is defined as follows:
\begin{eqnarray*} r &=& \left( \nxt[ a_1, a_1 ] + \nxt[ 0, 0 ] \right) \ / \ \cdots \ / \ \left( \nxt[ a_n, a_n ] + \nxt[ 0, 0 ] \right) 
\end{eqnarray*}
Notice that \ctpg $\C$, expression $r$ in $\Lonepp$ and tuple $(v,0,v,S)$ can be computed in polynomial time in the sizes of $A$ and $S$. Besides, it is straightforward to prove that $(v, 0, v, S) \in \semp{r}{\C}$ if and only if there exists $A' \subseteq A$ such that $\sum_{a \in A'} a = S$. This concludes the of $\np$-hardness of $\tupleeval(\Lonepp)$.
%\begin{itemize}
%\item[($\Leftarrow$)] %For the if part, 
%Suppose that there exists $A' \subseteq A$ such that $\sum_{a \in A'} a = S$, and assume that $A' = \{ a_{i_1}, \dots a_{i_m} \}$, for $1 \leq i_1 < \dots < i_m \leq n$.
%
%It is easy to see that $(v, t, v, t + a_i) \in \semp{\nxt[a_i, a_i]}{\C}$, and $(v, t, v, t) \in \semp{\nxt[0, 0]}{\C}$ whenever $t$ and $t + a_i$ are in $\Omega$, so in such case, both $(v, t, v, t + a_i)$ and $(v, t, v, t)$ are in $\semp{(\nxt[a_i, a_i] + \nxt[0, 0])}{\C}$. Hence, by concatenating these expressions, we also get that
%\[ (v, t, v, t + a_{i_k}) \in \semp{( \nxt [a_{i_j}, a_{i_j}] + \nxt[0, 0] ) \ / \ \dots \ / \ ( \nxt [a_{i_k}, a_{i_k}] + \nxt[0, 0] ) }{\C}\]
%since $(v, t, v, t) \in \semp{( \nxt [a_{i_l}, a_{i_l}] + \nxt[0, 0] )}{\C}$ for each $l \in \{j, %\ldots, k-1\}$, and $(v, t, v, t + a_{i_k}) \in \semp{ ( \nxt [a_{i_k}, a_{i_k}] + \nxt[0, 0] ) }{\C}$.
%
%In particular, this means that $(v, 0, v, a_{i_1}) \in \semp{\left( \nxt [a_1, a_1] + \nxt[0, 0] \right) \ / \ \dots \ / \ \left( \nxt [a_{i_1}, a_{i_1}] + \nxt[0, 0] \right)}{\C}$, and that for each $j \in \{1, \dots, m-1\}$, $(v, \sum_{k = 1}^{j} a_{i_k}, v, \sum_{k = 1}^{j + 1} a_{i_k}) \in \semp{( \nxt [a_{i_j}, a_{i_j}] + \nxt[0, 0] ) \ / \ \dots \ / \ ( \nxt [a_{i_{j+1}}, a_{i_{j+1}}] + \nxt[0, 0] )}{\C}$.
%
%Altogether, this implies that $(v, 0, v, \sum_{k=1}^m a_{i_k}) \in \semp{\left( \nxt [a_1 a_1 + \nxt[0, 0] \right) \ / \ \dots \ / \ \left( \nxt [a_{i_m}, a_{i_m}] + \nxt[0, 0] \right)}{\C}$. Finally, since we also have that $(v, t, v, t) \in \semp{\left(\nxt[a_{i_m}, a_{i_m}] + \nxt[0, 0] \right) \ / \ \dots \ / \ \left( \nxt[ a_m, a_m ] + \nxt[0, 0] \right)}{\C}$ and $\sum_{k=1}^m a_{i_k} = \sum_{a \in A'} a = S$, we get that $(v, 0, v, S) \in \semp{r}{\C}$.
%
%\item[($\Rightarrow$)]
%Now, for the only if part, suppose that $(v, 0, v, S) \in \semp{r}{\C}$. This implies that there exist time points $t_1, \dots, t_{n-1}$ such that $(v,0, v, t_1) \in \semp{(\nxt [a_1, a_1] + \nxt [0, 0])}{\C}$, $(v, t_i, v, t_{i+1}) \in \semp{(\nxt [a_{i+1}, a_{i+1}] + \nxt [0, 0])}{\C}$ for $i \in \{ 1, \dots, n-2 \}$, and $(v, t_{n-1}, v, S) \in \semp{(\nxt[a_n, a_n] + \nxt[0, 0])}{\C}$. Just as before, this means that $t_1$ is equal to either $0$ or $a_1$, $t_{i+1}$ is equal to either $t_i + a_{i+1}$ or $t_i$ for each $i$, and $S$ is equal to either $t_{n-1}$ or $t_{n-1} + a_n$.
%
%It is then easy to show by induction that, if we define $t_0 = 0$ and $t_n = S$, then for $i \in \{1, \dots, n-1\}$ we have that:
%\[ t_{i + 1} = \sum_{k=0}^{i} \left( t_{k + 1} - t_k \right) \]
%
%The base case is given by showing that $t_1 = t_1 - t_0 = t_1 - 0$, whereas if we suppose that, for some $i \leq n-2$, we have that:
%\[ t_{i + 1} = \sum_{k=0}^{i} \left( t_{k + 1} - t_k \right), \]
%then we get that
%\begin{align*}
%    t_{i + 2} & = \ t_{i + 2} - t_{i + 1} + t_{i + 1} \\
%        & = \ (t_{i + 2} - t_{i + 1}) + \sum_{k=0}^{i} \left( t_{k + 1} - t_k \right) \\
%        & = \ \sum_{k=0}^{i + 1} \left( t_{k + 1} - t_k \right)
%\end{align*}
%
%Finally, recall that $t_{k+1} - t_k$ is always either $0$ or $a_{k+1}$. Since this result implies that $S = \sum_{k=0}^{n-1} \left( t_{k + 1} - t_k \right)$ for the particular case where $i = n - 1$, we can define $A' = \{ t_{k + 1} - t_k \ \mid \ k \in \{ 0, \dots, n - 1 \} \} \setminus \{ 0 \}$ that satisfies both that $A' \subseteq A$ and that $\sum_{a \in A'} a = S$, completing the proof for \np-hardness.
%\end{itemize}

To show that this problem is \np-complete, it only remains to show that the problem is also in \np. We present a nondeterministic algorithm that works in polynomial time, $\textsc{TupleEvalSolve\_ANOI}$, that, given a \ctpg $\C$, an expression $r$ in $\Lonepp$ and a pair of temporal objects $(o_1, t_1, o_2, t_2)$, has a run that returns $\true$ if and only if $(o, t, o', t') \in \semp{r}{\C}$. This procedure is presented in Algorithm \ref{algo:ANOI}.

\LinesNumbered

\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Initialization}{Initialization}
    \Input{\ A \ctpg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, an expression $r$ in $\Lonepp$ and a pair of temporal objects $\left( o_1, t_1, o_2, t_2 \right)$}
    \Output{\ $\true$ if $\left( o, t, o', t' \right) \in \semp{r}{\C}$}
    \uIf{$r$ is a $\test$}{
        \uIf{$(o_1, t_1) \neq (o_2, t_2)$}{
            \Return $\false$
        }
        \uElseIf{$r = \vd$}{
            \Return $(o_1 \in N)$
        }
        \uElseIf{$r = \ed$}{
            \Return $(o_1 \in E)$
        }
        \uElseIf{$r = \ell$ for some \ $\ell \in \Lab$}{
            \Return $(\lambda(o_1) = \ell)$
        }
        \uElseIf{$r = \propt{p}{v}$ for some $p\in \Prop$ \ \text{and} $v\in \Val$}{
            \ForEach{valued interval $(v', I) \in \sigma(o_1, p)$}{
                \uIf{$t_1 \in I$}{
                    \Return $v' = v$
                }
            }
            \Return $\false$
        }
        \uElseIf{$r \, = \, < \mt$ with $\mt \in \Omega$}{
            \Return $(t_1 < \mt)$
        }
        \uElseIf{$r = \ex$}{
            \ForEach{interval $I \in \xi(o_1)$}{
                \uIf{$t_1 \in I$}{
                    \Return $\true$
                }
            }
            \Return $\false$
        }
        \uElseIf{$r = (\test_1 \vee \test_2)$}{
            \Return $\textsc{TupleEvalSolve}\left(\C,  (o_1, t_1, o_1, t_1), \test_1 \right)$ \textbf{or} $\textsc{TupleEvalSolve}\left(\C, (o_1, t_1, o_1, t_1), \test_2 \right)$
        }
        \uElseIf{$r   = (\test_1 \wedge \test_2)$}{
            \Return $\textsc{TupleEvalSolve}\left(\C, (o_1, t_1, o_1, t_1), \test_1 \right)$ \textbf{and} $\textsc{TupleEvalSolve}\left(\C, (o_1, t_1, o_1, t_1), \test_2 \right)$
        }
        \uElseIf{$r  = \left( \neg r' \right)$}{
            \Return \textbf{not} $ \textsc{TupleEvalSolve}\left(\C, (o_1, t_1, o_1, t_1), r' \right)$
        }
    }
    \uElseIf{$r = \nxt$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ t_2 = t_1 + 1
        \right)$
    }
    \uElseIf{$r = \prv$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ t_2 = t_1 - 1
        \right)$
    }
    \uElseIf{$r = \fw$}{
        \Return $\left(
            t_1 = t_2 \ \textbf{and} \ \left(
                \left( o_1 \in E \ \textbf{and} \ o_2 = \tgt\left( o_1 \right) \right)
                \ \textbf{or} \
                \left( o_2 \in E \ \textbf{and} \ o_1 = \src\left( o_2 \right) \right)
            \right)
        \right)$
    }
    \uElseIf{$r = \bw$}{
        \Return $\left(
            t_1 = t_2 \ \textbf{and} \ \left(
                (o_1 \in E \ \textbf{and} \ o_2 = \src(o_1))
                \ \textbf{or} \
                (o_2 \in E \ \textbf{and} \ o_1 = \tgt(o_2))
            \right)
        \right)$
    }
    \caption{$\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_2, t_2), r)$ (part I)}
    \label{algo:ANOI}
\end{algorithm}

$\textsc{TupleEvalSolve\_ANOI}$
%It is easy to see that the algorithm 
is very similar to $\textsc{TupleEvalSolve}$, so we will not discuss in detail what it does.
%that it does what is expected. 
Instead, we give an intuition of what the differences are that allow to return the right answer in non-deterministic polynomial time, instead of polynomial space.
First, notice that if $r$ is a test, then the algorithm works by solving basic tests efficiently,
%by their definition, 
and then conjunctions, disjunctions and negations of tests are solved just by using directly the definition of these Boolean connectives. Hence,
%as in boolean logic, so 
unlike what happens in the presence of path conditions, where we can have nested expressions with existential conditions and negations of existential conditions, sub-expressions for tests are efficiently solved by $\textsc{TupleEvalSolve\_ANOI}$.
%solvable.
Second, notice that for spatial navigation, we write the problem in terms of the reachability problem for graphs in a number of steps in a set $\{n, \ldots, m\}$.
%to $m$ steps in a graph. 
This problem can be efficiently solved by using exponentiation by squaring on the adjacency matrix. Besides, notice that for spatial navigation expressions in $\Lonepp$, we need to consider as many new objects as there are in $V \cup E$ since the time is fixed, which is why expressions $\fw[n, \_]$ and $\bw[n, \_]$ are equivalent to $\fw[n, m]$ and $\bw[n, m]$, respectively, with $m = n + |N \cup E| = n + |N| + |E|$.
Finally, polynomial time executions are ensured by the non-deterministic guess for $(o', t')$ in Line $64$, and the fact that the depth of the recursion tree is linear 
%height 
with respect to the size of the input expression $r$.
In particular, we do a single non-deterministic guess in Line $64$,
%, since this can be done in a single %nondeterministic 
%guess, 
instead of an exponential number of attempts (with respect to the size of the representation of $\Omega$) that would be necessary to find the right pair $(o', t')$ in a deterministic algorithm.

%Notice that if $r$ is any basic test ($\vd$, $\ed$, $\ell$, $\propt{p}{v}$, $<k$ or $\ex$), then if $(o_1, t_1) \neq (o_2, t_2)$, we will have both that $(v_1, t_1, v_2, t_2) \notin \semp{r}{\C}$ and that the algorithm will return $\false$ in line $3$ deterministically. Hence, assume that $(o_1, t_1) = (o_2, t_2)$. As the reader can easily verify, for each of these cases, the algorithm exactly checks whether $(o_1, t_1) \models r$ in polynomial time, so the property holds.

%Similarly, whenever $r$ is one of the navigation operators $\nxt$, $\prv$, $\fw$ or $\bw$, the algorithm checks exactly whether their definition for the given pair, \textit{i.e.}, object equality with the corresponding time adjacency for temporal navigation, and time equality with the corresponding object adjacency for spatial navigation.

%For the inductive case, suppose that, for any pair of temporal objects $(o_1, t_1, o_2, t_2) \in \Pt[\G]$ and expression $r$ in $\Lthree$, if $r$ has parsing tree of height $k$, then $\textsc{TupleEvalSolve\_ANOI}(\C, r, (o_1, t_1, o_2, t_2))$ has an execution returning $\true$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. We will show that if the height of $r$ is $k + 1$, it still holds that $\textsc{TupleEvalSolve\_ANOI}(\C, r, (o_1, t_1, o_2, t_2))$ has an execution returning $\true$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$.

\begin{algorithm}
%    \ContinuedFloat
    \SetAlgoLined
    \setcounter{AlgoLine}{35}
    \uElseIf{$r = \nxt[n, m]$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ n \leq (t_2 - t_1) \leq m
        \right)$
    }
    \uElseIf{$r = \prv[n, m]$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ n \leq (t_1 - t_2) \leq m
        \right)$
    }
    \uElseIf{$r = \fw[n, m]$}{
        \uIf{$t_1 \neq t_2$}{
            \Return $\false$
        }
        \uElse{
            Let $G = (N', E')$ be the graph where: \\
            \begin{itemize}
                \item $N' = (N \cup E)$
                \item $E' = \{
                    (v, e) \in N \times E \ \vert \ \src(e) = v
                \} \cup \{ 
                    (e, v) \in E \times N \ \vert \ \tgt(e) = v
                \}$
            \end{itemize}
            \Return $o_2$ is reachable from $o_1$ in $k$ steps in $G$, where $k \in \{n, \ldots, m\}$
        }
    }
    \uElseIf{$r = \bw[n, m]$}{
        \uIf{$t_1 \neq t_2$}{
            \Return $\false$
        }
        \uElse{
            Let $G = (N', E')$ be the graph where: \\
            \begin{itemize}
                \item $N' = (N \cup E)$
                \item $E' = \{
                    (v, e) \in N \times E \ \vert \ \tgt(e) = v
                \} \cup \{ 
                    (e, v) \in E \times N \ \vert \ \src(e) = v
                \}$
            \end{itemize}
            \Return $o_2$ is reachable from $o_1$ in $k$ steps in $G$, where $k \in \{n, \ldots, m\}$
        }
    }
    \uElseIf{$r = \nxt[n, \_]$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ n \leq (t_2 - t_1)
        \right)$
    }
    \uElseIf{$r = \prv[n, \_]$}{
        \Return $\left(
            o_1 = o_2 \ \textbf{and} \ n \leq (t_1 - t_2)
        \right)$
    }
    \uElseIf{$r = \fw[n, \_]$}{
        %\uIf{$t_1 \neq t_2$}{
        %    \Return $\false$
        %}
        %\uElse{
            $m \gets n + |N| + |E|$ \\
%            Let $G = (N', E')$ be the graph where: \\
%            \begin{itemize}
%                \item $N' = (N \cup E)$
%                \item $E' = \{
%                    (v, e) \in N \times E \ \vert \
%                    \src(e) = v
%                \} \cup \{ 
%                    (e, v) \in E \times N \ \vert \
%                    \tgt(e) = v
%                \}$
%            \end{itemize}
            \Return $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_2, t_2), \fw[n,m])$
            %Reachability from $o_1$ to $o_2$ in $n$ to $m$ steps on $G$
        %}
    }
    \uElseIf{$r = \bw[n, \_]$}{
        %\uIf{$t_1 \neq t_2$}{
        %    \Return $\false$
        %}
        %\uElse{
            $m \gets n + |N| + |E|$ \\
            %Let $G = (N', E')$ be the graph where: \\
            %\begin{itemize}
            %    \item $N' = (N \cup E)$
            %    \item $E' = \{
            %        (v, e) \in N \times E \ \vert \ \tgt(e) = v
            %    \} \cup \{ 
            %        (e, v) \in E \times N \ \vert \ \src(e) = v
            %    \}$
            %\end{itemize}
            \Return          $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_2, t_2), \bw[n,m])$
            %Reachability from $o_1$ to $o_2$ in $n$ to $m$ steps on $G$
        %}
    }
    \uElseIf{$r = (r_1 + r_2)$}{
        %Nondeterministicall 
        Guess $i \in \{ 1, 2 \}$ \\
        \Return $\textsc{TupleEvalSolve\_ANOI}(\C, ( o_1, t_1, o_2, t_2), r_i)$
    }
    \uElseIf{$r = (r_1 \ / \ r_2)$}{
        %Nondeterministically 
        Guess $(o', t') \in (N \cup E) \times \Omega$ \\
        \Return $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o', t'), r_1)$ \textbf{and}  $\textsc{TupleEvalSolve\_ANOI}(\C, (o', t', o_2, t_2), r_2)$ \\
    }
    \caption{$\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_2, t_2), r)$ (part II)}
\end{algorithm}

%First suppose that $r$ is a test. We know that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ only if $(o_1, t_1) = (o_2, t_2)$. As before, if $(o_1, t_1) \neq (o_2, t_2)$, the algorithm returns $\false$ in line $3$, else we go case by case.

%If $r$ is a conjunction of tests, $(\test_1 \wedge \test_2)$, then $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$ if and only if both $(o_1, t_1) \models \test_1$ and $(o_1, t_1) \models \test_2$. This is equivalent to having, $(o_1, t_1, o_1, t_1) \in \semp{\test_1}{\C}$ and $(o_1, t_1, o_1, t_1) \in \semp{\test_2}{\C}$. Notice then that by induction hypothesis, the first condition holds if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_1)$ has an execution returning $\true$, and the second condition holds if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_2)$. Thus, if $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$, we have both calls having executions returning $\true$, so the conjunction will be $\true$ as well. In contrast, when $(o_1, t_1, o_1, t_1) \notin \semp{r}{\C}$, then either $(o_1, t_1, o_1, t_1) \notin \semp{\test_i}{\C}$ for either $i = 1$ or $i = 2$. In any case, the respective call $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_i)$ will have no execution returning $\true$ and the conjunction will be $\false$.

%If $r$ is a disjunction of tests, $(\test_1 \vee \test_2)$, then $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$ if and only if either $(o_1, t_1) \models \test_1$ or $(o_1, t_1) \models \test_2$. This is equivalent to having that either $(o_1, t_1, o_1, t_1) \in \semp{\test_1}{\C}$ or $(o_1, t_1, o_1, t_1) \in \semp{\test_2}{\C}$. Notice then that by induction hypothesis, the first condition holds if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_1)$ has an execution returning $\true$, and the second condition holds if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_2)$. Thus, if $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$, we will have that for either $i = 1$ or $i = 2$, $(o_1, t_1, o_1, t_1) \in \semp{\test_i}{\C}$, so  $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_i)$ will return $\true$, and the disjunction will be $\true$ as well. In contrast, when $(o_1, t_1, o_1, t_1) \notin \semp{r}{\C}$, then $(o_1, t_1, o_1, t_1) \notin \semp{\test_i}{\C}$ for both $i = 1$ and $i = 2$. In any case, the respective call $\textsc{TupleEvalSolve\_ANOI}(\C, (o_1, t_1, o_1, t_1), \test_i)$ will have no execution returning $\true$, so any execution will be returning $\false \textbf{or} \false$, \textit{i.e.}, $\false$.

% If $r$ is a negation of a test, $(\neg \test)$, then $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$ if and only if $(o_1, t_1) \not\models \test$. This is equivalent to having, $(o_1, t_1, o_1, t_1) \notin \semp{\test}{\C}$. Since $\test$ has parsing tree of height $k$, then $(o_1, t_1, o_1, t_1) \notin \semp{\test}{\C}$ if and only if all executions of $\textsc{TupleEvalSolve\_ANOI}(\C, \test, (o_1, t_1, o_1, t_1))$ return $\false$. Although the algorithm is nondeterministic, notice that since $\Lonepp$ has no path conditions, the recursion is completely deterministic on tests, so this happens if and only if the (deterministic unique) execution of  $\textsc{TupleEvalSolve\_ANOI}(\C, \test, (o_1, t_1, o_1, t_1))$ returns $\false$. Since the algorithm returns the negation of this call, we get that $(o_1, t_1, o_1, t_1) \in \semp{r}{\C}$ if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, r, (o_1, t_1, o_1, t_1))$ returns $\true$.

% If $r$ is an ANOI expression of the form $\nxt[n, m]$, notice that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists $i \in [n, m]$ such that $(o_1, t_1, o_2, t_2) \in \semp{\nxt^i}{\C}$, \textit{i.e.}, if and only if $o_1 = o_2$ and $t_2 = t_1 + i$. This is equivalent to having the equality $o_1 = o_2$ and $t_2 - t_1 \in [n, m]$, which is exactly what the algorithm returns for this case.

% If $r$ is an ANOI expression of the form $\prv[n, m]$, notice that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists $i \in [n, m]$ such that $(o_1, t_1, o_2, t_2) \in \semp{\prv^i}{\C}$, \textit{i.e.}, if and only if $o_1 = o_2$ and $t_2 = t_1 - i$. This is equivalent to having the equality $o_1 = o_2$ and $t_1 - t_2 \in [n, m]$, which, again, is exactly what the algorithm returns for this case.

% If $r$ is an ANOI expression of the form $\fw[n, m]$, we know that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists $i \in [n, m]$ such that $(o_1, t_1, o_2, t_2) \in \semp{\fw^i}{\C}$. This is something similar to reachability in $n$ to $m$ steps in a graph, except that here one step is moving from a (source) node to an edge, or from an edge to a (target) node. Thus, an equivalent graph is built from $N$, $E$ and $\rho$ to have the proper reduction that works in polynomial time and that is equivalent to the condition.

% If $r$ is an ANOI expression of the form $\bw[n, m]$, the algorithm acts very similarly, except that now we want backwards reachability, so the graph is build using the backwards edges of the one mentioned below to test whether $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$.

% The ANOI expressions of the form $\nxt[n, \_]$ and $\prv[n, \_]$ work just as $\nxt[n, m]$ and $\prv[n, m]$, except that instead of checking that $(t_2 - t_1) \in [n, m]$ and $(t_1 - t_2) \in [n, m]$ respectively, we check that $(t_2 - t_1) \geq n$ and $(t_1 - t_2) \geq n$.

% The ANOI expressions of the form $\fw[n, \_]$ and $\bw[n, \_]$, in turn, work just as $\fw[n, m]$ and $\bw[n, m]$ above, but for $m = n + (|N \cup E||\Omega|)^2$, as we know that $\semp{\fw[n, \_]}{\C} = \semp{\fw[n, m]}{\C}$ and $\semp{\bw[n, \_]}{\C} = \semp{\bw[n, m]}{\C}$ for this value for $m$, as already shown for some of the previous theorems.

% \pedro{Marcelo: If you reach this, please let me know if it is clear enough or if I should specify how to do (using something similar to exponentiation by squaring) reachability in $n$ to $m$ steps in a normal graph, or even give stronger arguments on why the problems are equivalent.}

% Finally, there are two nondeterministic recursive cases. The first if for expressions $r = (r_1 + r_2)$ where $r_1$ and $r_2$ are also expressions in the language. In this case, we know that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if $(o_1, t_1, o_2, t_2) \in \semp{r_i}{\C}$ for either $i = 1$ or $i = 2$, which, by induction, happens if and only if $\textsc{TupleEvalSolve\_ANOI}(\C, r_i, (o_1, t_1, o_2, t_2)$ has an execution returning $\true$ for either $i = 1$ or $i = 2$. Suppose then that $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$. Without loss of generality, suppose that this means that for $i = 1$, $\textsc{TupleEvalSolve\_ANOI}(\C, r_i, (o_1, t_1, o_2, t_2)$ has an execution returning $\true$. Then the execution that uses the said execution in line $75$ and guesses $i = 1$ in line $74$ returns $\true$. Oppositely, if  $(o_1, t_1, o_2, t_2) \notin \semp{r}{\C}$, then for both $i = 1$ and $i = 2$, the execution $\textsc{TupleEvalSolve\_ANOI}(\C, r_i, (o_1, t_1, o_2, t_2)$ no execution will return $\true$, so no matter what value for $i$ is guessed at line $74$, all executions will return $\false$.

% The second nondeterministic case if for expressions $r = (r_1 \ / \ r_2)$. By definition of concatenation, $(o_1, t_1, o_2, t_2) \in \semp{r}{\C}$ if and only if there exists a temporal object $(o', t')$ such that $(o_1, t_1, o', t') \in \semp{r_1}{\C}$ and $(o', t', o_2, t_2) \in \semp{r_2}{\C}$. By induction, this happens if and only if there exists a temporal object $(o', t')$ such that $\textsc{TupleEvalSolve\_ANOI}(\C, r_1, (o_1, t_1, o', t')$ and $\textsc{TupleEvalSolve\_ANOI}(\C, r_2, (o', t', o_2, t_2)$ have executions that returns $\true$. Suppose then that such temporal object exists. Then the execution that guesses this temporal object in line $77$, and then uses the executions that return $\true$ for the recursive calls will return $\true$. Oppositely, if no such temporal object exists, then no matter what temporal object is chosen at line $77$, either all executions for $\textsc{TupleEvalSolve\_ANOI}(\C, r_1, (o_1, t_1, o', t')$ or all executions for $\textsc{TupleEvalSolve\_ANOI}(\C, r_2, (o', t', o_2, t_2)$ will return $\false$. In any case, this means that the algorithm will return $\false$, which completes the induction proof.

% To complete the proof of the theorem, we show that the whole algorithm works in polynomial time. To show this, notice that the height of the recursion tree is polynomial, since there only are as many recursive calls as the number of expressions in the parsing tree for $r$, which is $O(\| r \|)$.

% Furthermore, tests are solved in deterministic polynomial time since all basic tests are polynomial and solving conjunctions, disjunctions or negations of tests comes down to evaluating a boolean formula, which can be done in linear time with respect to the size of the formula, which here is $O(\| r \|)$.

% Testing (single step) temporal and spatial navigation is also clearly polynomial, whereas ANOI expressions can also be evaluated in polynomial time, since time navigation is trivially feasible in polynomial time, the graphs that are built have polynomial size with respect to the size of the input, the representation of $m = (|(N \cup E)| \cdot |\Omega|)^2$ also has polynomial size with respect to the size of the input, and reachability in $n$ to $m$ steps can be done in polynomial time, using exponentiation by squaring algorithms.

% Finally, polynomial time is preserved for the nondeterministic executions for expressions of the form $(r_1 + r_2)$ and $(r_1 \ / \ r_2)$ since only $O(\|r\|)$ recursive calls are executed, nondeterministic guesses take a single step and then the computation of the result from the recursive calls is straightforward.

%\pedro{A single step in this algorithm, but virtually a polynomial number of guesses in a Turing machine, should I make this clear?}

%\qed


==> proof_t5.tex <==
\subsection{Proof of Theorem \ref{th:LthreepTupleNP}}
\label{proof:LthreepTupleNP}

Notice that every expression in $\Lthreep$ is also an expression in $\Lthree$, so \pspace-membership follows immediately from Theorem \ref{th:LthreeTuplePSPACE}.
%for the problem $\tupleeval(\Lthreep)$. 
Hence, we only need to prove \pspace-hardness for $\Lthreep$.

To show this, we replace test expressions $r_i$ in the proof in Section \ref{proof:LthreeTuplePSPACE} 
%for theorem \ref{th:LthreeTuplePSPACE}, 
by an 
%alternative test 
expression in $\Lthreep$ that will be 
denoted by $q_i$. %These 
Expression $q_i$ is defined in such a way that,
%will be such that, 
for every time $t$, it holds that $(v, t, v, t) \in \semp{q_i}{\C}$ if and only if $(v, t, v, t) \in \semp{r_i}{\C}$, \textit{i.e.}, if and only if $\bit(i, t)$ is $\true$, where $\bit(i, t)$ holds if the $i$-th bit of time $t$ (from right to left when written in its binary representation) is 1. More precisely,
expression $q_i$ %are 
is defined as follow:
\begin{eqnarray*}
    q_i &  = & ?\left(
        \left(
            ( \prv[0, 0] + \prv[2^n, 2^n] ) \ / \
            \ldots \ / \
            %\left( \prv[0, 0] + \prv[2^{i+1}, 2^{i+1}] \right) \ / \
            ( \prv[0, 0] + \prv[2^i, 2^i] )
        \right) \ / \ \left(
            < 2^i \wedge \neg < 2^{i-1}
        \right)
    \right)
\end{eqnarray*}
Notice that the length of the representation $2^k$ is $k$, so the whole expression $q_i$ has length $O(n^2)$, which is polynomial with respect to the size of $\psi$. Also, notice that as before, we only need a polynomial number of these expressions for the reduction, and no further nesting of numerical occurrence indicators is required for the proof. Hence, we only need to prove that $(v, t, v, t) \in \semp{q_i}{\C}$ if and only if $\bit(i, t)$ is $\true$.
%
Recall that for this reduction, $\C$ is a \ctpg consisting of only one node $v$, existing from time $0$ to time $2^n-1$, with no edges or properties, so %keep in mind that 
any temporal object considered will be of the form $(v,t)$.
%have object $v$.

First, notice that $q_i$ is a path test, so $(v, t, v, t) \in \semp{q_i}{\C}$ if and only if there exists a time point $t'$ such that
\begin{eqnarray*}
    (v, t, v, t') &  \in & \semp{\left(
        ( \prv[0, 0] + \prv[2^n, 2^n] ) \ / \
        \ldots \ / \
        %\left( \prv[0, 0] + \prv[2^{i+1}, 2^{i+1}] \right) \ / \
        ( \prv[0, 0] + \prv[2^i, 2^i] )
    \right) \ / \ \left(
        < 2^i \wedge \neg < 2^{i-1}
    \right)}{\C}
\end{eqnarray*}
As in \textbf{Step 1} of Section \ref{proof:LthreeTuplePSPACE}, since the last part of the expression is a test, this is equivalent to the existence of a time point $t'$ such that $(v, t') \models \left( < 2^i \wedge \neg < 2^{i-1} \right)$, \textit{i.e.}, the $i$-th bit of $t'$ is $1$ and
\begin{eqnarray}\label{eq-qi-int}
    (v, t, v, t') &  \in & \semp{
        ( \prv[0, 0] + \prv[2^n, 2^n] ) \ / \
        %\left( \prv[0, 0] + \prv[2^{i+1}, 2^{i+1}] \right) \ / \
        \ldots \ / \ ( \prv[0, 0] + \prv[2^i, 2^i] )
    }{\C}
\end{eqnarray}
We now prove that $(v, t, v, t) \in \semp{q_i}{\C}$ if and only if $\bit(i, t)$ is $\true$.
To show direction ($\Leftarrow$), suppose that $\bit(i, t)$ is $\true$. Notice then that $(v, t_1, v, t_2) \in \semp{( \prv[0, 0] + \prv[2^k, 2^k])}{\C}$, if and only if $t_2 = t_1$ or $t_2 = t_1 - 2^k$. In particular, if the $(k+1)$-th bit of $t_1$ is $1$, then $t_2 = t_1 - 2^k$ has a binary representation that is equal to that of $t_1$ except on the $(k+1)$-th bit,
%where a $0$ is instead, 
and $(v, t_1, v, t_2) \in \semp{( \prv[0, 0] + \prv[2^k, 2^k] )}{\C}$. Similarly, if the $(k+1)$-th bit of $t_1$ is $0$, then $t_2 = t_1$ has a binary representation that is equal to that of $t_1$, %with a $0$ on the $k + 1$-th bit, 
and also $(v, t_1, v, t_2) \in \semp{( \prv[0, 0] + \prv[2^k, 2^k])}{\C}$.
%
As in Section \ref{proof:LthreeTuplePSPACE}, given $b \in \{\true, \false\}$, let $\mathbbm{1}_b$ be $1$ if $b = \true$, and be $0$ otherwise. Moreover, define the sequence of time points $t_{n+1}, \dots, t_i$ such that $t_{n+1} = t$ and $t_k = t_{k + 1} - \mathbbm{1}_{\bit(k + 1, t)} \cdot 2^k$ for $k \in \{ i, \dots, n \}$. 
Then for every $k \in \{ i, \dots, n \}$, it holds that 
$(v, t_k, v, t_{k+1}) \in \semp{( \prv[0, 0] + \prv[2^k, 2^k] )}{\C}$, and in particular, $t' = t - \sum_{k=i}^n \mathbbm{1}_{\bit(k + 1, t)} \cdot 2^k$ satisfies \eqref{eq-qi-int}.
%
%{\color{red}
Therefore, 
%Furthermore, by construction, $t'$ is equal to $t \mod 2^i$, so 
if the $i$-th bit of $t$ is $1$, then the $i$-th bit of $t'$ will be 1 as well.
%also will. 
Hence, given $\bit(i, t)$ is $\true$, we conclude that $(v, t, v, t) \in \semp{q_i}{\C}$, since for $t' = t - \sum_{k=i}^n \mathbbm{1}_{\bit(k + 1, t)} \cdot 2^k$, equation \eqref{eq-qi-int} holds and $(v,t') \models (< 2^i \wedge \neg < 2^{i-1})$.
%and $t \mod 2^i$ is trivially smaller than $2^i$, and greater than $2^{i-1}$ for having a $1$ as its $i$-th bit.}

To show direction ($\Rightarrow$), suppose that $(v, t, v, t) \in \semp{q_i}{\C}$. Then there exists a time point $t'$ such that \eqref{eq-qi-int} holds, which only holds if there exists a sequence of time points $t_{n+1}, \dots, t_i$ where $t_{n+1} = t$ and either $t_k = t_{k + 1}$ or $t_k = t _{k + 1} - 2^k$ for $k \in \{ i, \dots, n \}$, and $t_i = t'$. Notice that for such values for $k$, $2^k$ is a multiple of $2^i$, so $t' = t + d \cdot 2^i$ for some integer $d$. %\textit{i.e.}, $t' \mod 2^i = t \mod 2^i$, 
We conclude that the $i$-th bit of $t$ is equal to $1$ if and only if the $i$-th bit of $t'$ is equal to $1$. Moreover, $(v, t') \models ( < 2^i \wedge \neg < 2^{i-1})$, so the $i$-th bit of $t'$ is indeed equal to $1$, so $\bit(i, t)$ must be equal to $\true$.

From the previous paragraphs, we conclude that $(v, t, v, t) \in \semp{q_i}{\C}$ if and only if $\bit(i, t)$ is $\true$. Hence, by replacing $r_i$ with $q_i$ in the proof of Theorem \ref{th:LthreeTuplePSPACE}, we deduce that $\Lthreep$ is also \pspace-hard, which was to be shown.

==> z_2examples.tex <==
Consider Figure~\ref{fig:g1} that depicts an interaction network.  Note that vertices and edges have associated properties, and that they each are associated with a time interval.  We will refer to a pair of spatially adjacent vertices as \emph{neighbors}.  We may be interested in learning the following information about this network:

\input{t1}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figs/g1.pdf}
\caption{\tg $\G$ \julia{revise, make intervals closed-closed}}
\label{fig:g1}
\end{figure}

\begin{enumerate}
    \item What are the paths in $\G$ such that all components in the path (vertices and edges) exist at the same time?  In our example, these are from Ann to Bob via $e_1$ during the interval $[2,6]$, and from Bob to Cat via $e_2$ during the interval $[7, 8]$. (snapshot reducibility) \julia{Are we returning time-annotated matches?  If so, are using intervals to associate time with the generated paths?  It makes sense here, but not in the next example.}
    
    \item What are the  paths in $\G$ in which components (vertices and edges) are temporally-adjacent, and in which time increases along the path? In our example, there is one such path of length 3:  Ann@4 - $e_1$@5 - Bob@6 - $e_2$@7 - Cat@8.  There are also several paths of length 2 (from Ann to Bob, and from Bob to Cat).
    
    \item List all tuples $(v', v, v'')$ in which vertex $v$ has two temporally adjacent neighbors $v' \neq v''$ such that $v'$ occurs earlier than $v$ and $v''$ occurs later than $v$.  In our example, one such tuple is $(Ann@5, Bob@6, Cat@7)$.  Another is $(Ann@1, Bob@2, Cat@3)$.  \julia{1) Do we want to always return paths?  2) Is it reasonable to require that when two vertices are neighbors, that we also traverse an edge between them during one of the times of the times during which matching occurs?  If so, the first match is valid but the second is not because you cannot travel from Bob to Cat or from Cat to Bob at time 2 or at time 3.  3) Is it reasonable to leave the (spatial) direction of the edge unspecified?  Meaning, $v$ and $v'$ are neighbors when there is an edge from $v$ to $v'$ or from $v'$ to $v$.  Or is the notion of neighbor I have in mind syntactic sugar?}
    
    \item List all temporally-increasing (not necessarily temporally-adjacent) paths in which each edge exists for at least 2 consecutive time points.  \julia{stumbling on how to associate time with the path in the result to show what the output looks like, especially now that I'm explicitly asking for intervals; and point semantics is problematic here: if we have two paths in which some edge $e$ is associated with $[1,2]$ and with $[3,4]$, and all other elements of the path are the same, then the two paths would be coalesced, with $e=[1,4]$.}
    
    \item List all temporally-increasing paths in which there are temporal gaps of specific length between adjacent elements.
    
    \item (I want to go from city A to city B, taking a path from which there is a road to city C.)
\end{enumerate}

\julia{I'm convinced that it's natural to limit the expressiveness based on the types of temporal objects we want to return.  Always paths?  Always temporally-equivalent or adjacent, and spatially-equivalent or adjacent (otherwise it's not a path), and with every element associated with a single time point? If so, (4) above doesn't make sense.}



==> z_deprecated_proof.tex <==
 
In a very similar way, we will prove that $\patheval(\Lthree)$ is also in \pspace. For this, consider the analog algorithm below:
  
\LinesNumbered

\begin{algorithm}[H]
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \Input{A \coal \tg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, an expression $\pt$ in $\Lthree$ and a path $p \in \Pt[\C]$}
    \Output{$\true$ if and only if $p \in \sem{\pt}$}
    \uIf{$r = \nxt$}{
        \uIf{$length(p) \neq 2$}{
            \Return \false
        }
        $(o,t)(o',t) \gets p$ \\
        \Return $o = o' \ \wedge \ t' = t + 1$
    }
    \uElseIf{$r = \prv$}{
        \uIf{$length(p) \neq 2$}{
            \Return \false
        }
        $(o,t)(o',t) \gets p$ \\
        \Return $o = o' \ \wedge \ t' = t - 1$
    }
    \uElseIf{$r = \fw$}{
        \uIf{$length(p) \neq 2$}{
            \Return \false
        }
        $(o,t)(o',t) \gets p$ \\
        \Return $t = t' \ \wedge \ \left(
            \left( o \in E \ \wedge \ o' = tgt(o) \right)
            \vee
            \left( o' \in E \ \wedge \ o = src(o') \right)
        \right)$
    }
    \uElseIf{$r = \bw$}{
        \uIf{$length(p) \neq 2$}{
            \Return \false
        }
        $(o,t)(o',t) \gets p$ \\
        \Return $t = t' \ \wedge \ \left(
            \left( o \in E \ \wedge \ o = tgt(o') \right)
            \vee
            \left( o' \in E \ \wedge \ o' = src(o) \right)
        \right)$
    }
    \uElseIf{$r \ matches \ \test$}{
        \uIf{$length(p) \neq 1$}{
            \Return \false
        }
        $(o,t) \gets p$ \\
        \Return $TupleEvalSolve\left(\C, r, (o, t, o, t)\right)$
    }
    \uElseIf{$r$ matches $(\pt + \pt)$}{
        $(r_1 + r_2) \gets r$ \\
        Non-deterministically guess $i \in \lbrace 1, 2 \rbrace$ \\
        return $PathEvalSolve\left(\C, r_i, p \right)$
    }
    \uElseIf{$r$ matches $(\pt \ / \ \pt)$}{
        $(r_1 \ / \ r_2) \gets r$ \\
        Non-deterministically guess a temporal object $(o', t')$ in $p$ \\
        $(o_1, t_1) \cdots (o', t') \cdots (o_2, t_2) \gets p$ \\
        $b_1 \gets PathEvalSolve(\C, r_1, (o_1, t_1) \cdots (o', t'))$ \\
        $b_2 \gets PathEvalSolve(\C, r_2, (o', t') \cdots (o_2, t_2)$ \\
        \Return $b_1 \wedge b_2$
    }
    \uElseIf{$r$ matches $(\pt[n, m]$}{
        $r'[n, m] \gets r$ \\
        Non-deterministically guess $i \in [n, m]$ \\
        \ForEach{$j \in [0, i-1]$}{
            Non-deterministically guess a temporal object $(o', t')$ in $p$ \\
            $(o_1, t_1) \cdots (o', t') \cdots (o_2, t_2) \gets p$ \\
            \uIf{$\neg PathEvalSolve(\C, r', (o_1, t_1) \cdots (o', t'))$}{
                \Return \false
            }
            $p \gets (o', t') \cdots (o_2, t_2)$ \\
        }
        \Return $PathEvalSolve(\C, r', p)$
    }
    \uElseIf{$r$ matches $(\pt[n, \_]$}{
        $r'[n, \_] \gets r$ \\
        Non-deterministically guess $i \in [n, n + |\Omega| \cdot |V \cup E|]$ \\
        \ForEach{$j \in [0, i-1]$}{
            Non-deterministically guess a temporal object $(o', t')$ in $p$ \\
            $(o_1, t_1) \cdots (o', t') \cdots (o_2, t_2) \gets p$ \\
            \uIf{$\neg PathEvalSolve(\C, r', (o_1, t_1) \cdots (o', t'))$}{
                \Return \false
            }
            $p \gets (o', t') \cdots (o_2, t_2)$ \\
        }
        \Return $PathEvalSolve(\C, r', p)$
    }
    \caption{$PathEvalSolve\left(\C, r, p \right)$ (part I)}
    
\end{algorithm}

We will prove that the algorithm is in \npspace by showing that for every \coal \tg $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$, expression $r$ in $\Lthree$ and path $p \in \Pt[\C]$, $p \in \sem{r}$ if and only if there is an execution of algorithm $PathEvalSolve \left(\C, r, p \right)$ that returns $\true$ using only polynomial space.\\

Notice firstly that here again the algorithm is recursive, and that the depth of the recursion is polynomial, since at almost every step we call the algorithm, the size of the path expression strictly decreases, except for two cases. The first is when we check the existence of a path ($\pt = (?\pt')$), for which call the previous algorithm $TupleEvalSolve$, that we know is in \pspace. The second is when the algorithm ends because the path expression is a basic expression that cannot be further broken down. Notice too that, here, paths are also nonincreasing in length. Hence, the recursion tree has polynomial height.\\

Secondly, just as before, notice that at every step of the algorithm, we only need to store the result of one call at the time. Hence, at the most, we will need to have in memory as many calls to the algorithm as the recursion tree height. This number is polynomial, and since every non-recursive step is either a non-deterministic guess, a call that we already know is in \npspace to $TupleEvalSolve$ or a step clearly in polynomial time in the size of the input, we get that the whole algorithm gives an answer in \npspace. \\

Now, let  $\C = \left( \Omega, N, E, \rho, \lambda, \xi, \sigma \right)$ be a \coal \tg, let $r$ be an expression in $\Lthree$ and let $p \in \Pt[\C]$ be a path in $\C$. First suppose that $p$ is in $\sem{r}$. We will show by structural induction that there exists an execution of algorithm $TupleEvalSolve \left( \C, r, p \right) $ that returns $\true$.\\

Here, th four base cases given by when $\pt$ is equal to either $\nxt$, $\prv$, $\fw$ or $\bw$ can be easily checked by their definitions, since the algorithm tests exactly those underlying definitions, in a deterministic way. \\

Secondly, if the path expression $r$ is of the form $\test$, then we know that $p \in \sem{r}$ if $p$ is composed of a single temporal object $(o, t)$ and $(o, t)$ satisfies that test. Notice that this is exactly the same that is tested by $TupleEvalSolve(\C, r, (o, t, o, t)$, since as we proved, that call is $\true$ if and only if there exists a path from $(o, t)$ to $(o, t)$ satisfying $r$, and $r$ being a test, such path can only be $(o, t)$. \\

As for regular path expressions $r$ of the form $(r_1 + r_2)$ where $r_1$ and $r_2$ are also regular path expressions, this works exactly as before. We know that by definition $\sem{(r_1 + r_2)} = \sem{r_1} \cup \sem{r_2}$. Hence, if $p\in \sem{r}$, then either $p \in \sem{r_1}$ or $p \in \sem{\pt_2}$. In any case, we can non-deterministically guess the index $i \in \lbrace 1, 2 \rbrace$ such that $p \in \sem{r_i}$, and if the result of $PathEvalSolve \left(\C, r_i, p \right)$ will be $\true$ by induction, so the execution will return $\true$. \\

For regular path expressions $r$ of the form $(r_1 \ / \ r_2)$ where $r_1$ and $r_2$ are also regular path expressions, here again we know that if $p \in \sem{r}$, then there must exist a temporal object $(o',t') \in \Pt[\C]$ such that $p = (o_1, t_1) \cdots (o', t') \cdots (o_2, t_2)$ and both conditions $(o_1, t_1) \cdots (o', t') \in \sem{r_1}$ and $(o', t') \cdots (o_2, t_2) \in \sem{r_2}$ hold. Thus, by correctly guessing this particular temporal object $(o',t')$, we get that both $b_1 = TupleEvalSolve(\C, r_1, (o_1, t_1) \cdots (o', t'))$ and $b_2 = TupleEvalSolve(\C, r_2, (o', t') \cdots (o_2, t_2))$ will be $\true$, so the corresponding non-deterministic execution will return $b_1 \wedge b_2 = \true$.

Finally, for expressions $r$ matching regular expressions with numerical occurrence indicators of the form $r'[n, m]$ or $r'[n, \_]$, recall that, by definition, $\sem{r'[n, m]} = \bigcup_{k=n}^m \sem{r'^k}$ and $\sem{r'[n, \_]} = \bigcup_{k \geq n} \sem{r'^k}$. This implies that $p \in \sem{r'[n, m]}$ if and only if there exists an integer $k \in [n, m]$ such that $p \in \sem{r'^k}$. Respectively, $p \in \sem{r'[n, \_]}$ if and only if there exists an integer $k \geq n$ such that $p \in \sem{r'^k}$. As before, $k$ can be assumed to have polynomial size with respect to the size of the input, since at the most we will only be interested to do an additional step in the loop if it reaches a temporal object that has not been previously reached, so at the most $k_max = n + |V \cup E| \cdot |\Omega|$ steps, which can be encoded in size $\log k_max$, polynomial in the size of the input. In both cases, assume then that, at lines $39$ and $49$ respectively, we non-deterministically guess $i$ as this integer $k$. The whole following process is analogous to the one for $TupleEvalSolve$, except that we check for partial paths instead of pairs of temporal objects, by accurately choosing the right temporal object $(o', t')$ in $p$, so by the end, we will also get $\true$.

To finish the proof, it only remains to prove that, if $p \notin \sem{r}$ then \textbf{there is no execution} that will return $\true$, which we will show by structural induction as well. Assume then in the following that $p \notin \sem{r}$.

Firstly, basic cases of the form $\nxt$, $\prv$, $\fw$ and $\bw$ can be easily inspected by their respective definitions, since in every case we either have a path of a length that is not according to one of those basic cases or the definition doesn't hold, and all this is clearly done deterministicly.

As for the case when $r$ is a test, we already showed that the problem was equivalent to the one solved by $TupleEvalSolve$, so this will return $\false$. \\

As for expressions $r$ matching $(r_1 + r_2)$ for regular path expressions $r_1$ and $r_2$, if we supposed that we could guess $i \in \lbrace 1, 2 \rbrace$ such that $PathEvalSolve(\C, r_i, p) = \true$, by induction we would know that $p \in \sem{r_i}$, but $\sem{r_i} \subseteq \sem{(r_1 + r_2)}$, so this would also mean that $p \in \sem{r}$, which is a contradiction, so no execution will return $\true$.

Similarly, for expressions $r$ of the form $(r_1 \ / \ r_2)$ where $r_1$ and $r_2$ are also regular path expressions, if we supposed that we could guess a temporal object $(o', t')$ such that $b_1 \wedge b_2$ is $\true$, we would have that $PathEvalSolve(\C, r_1, (o_1, t_1) \cdots (o', t'))$ and $PathEvalSolve(\C, r, (o', t') \cdots (o_2, t_2))$ would have had returned $\true$, which in turn requires by induction the existence of a path $(o_1, t_1)\cdots (o',t) \in \sem{r_1}$ and a path $(o', t') \cdots (o_2, t_2) \in \sem{r_2}$. By definition of $\sem{(r_1 \ / \ r_2)}$ this implies that the concatenation of such paths $(o_1, t_1) \cdots (o',t') \cdots (o_2, t_2) = p$ actually belongs to $\sem{(r_1 \ / \ r_2)} = \sem{r}$, which is a contradiction too, and again, no execution will return $\true$.

Finally, for path expressions $r$ of the form $r'[n, m]$ or $r'[n, \_]$, if we were to guess an integer $i \geq n$ and a sequence of temporal objects such that we reach line $46$ or $56$ respectively returning $\true$, then that would mean that we would have found a sequence of $i + 1$ temporal objects such that, each consecutive pair of temporal objects $(o, t)$ and $(o', t')$ satisfies the call to $PathEvalSolve$ on the expression $r'$, since no call returned $\false$ on line $44$ or $54$ respectively. Notice too that lines $61$ and $71$ imply that every time we decompose $p$ into paths of the form $(o_1, t_1) \cdots (o', t') \cdots (o_2, t_2)$, we are taking a first part of path $p$ before $(o', t')$ and the rest of the path after $(o' t')$, so the concatenation of all partial paths checked is exactly $p$.

Hence, the whole process implies that the concatenation of such existing paths, \textit{i.e.}, $p$, belongs to $\sem{\pt^i}$, where $i \geq n$ and $i \leq m$ or $m \leq + \left| \Omega \right| \cdot \left| V \cup E \right|$ respectively, which by definition of $r'[n, m]$ and $r'[n, \_]$ means that $p \in \sem{r'[n, m]}$ or $p \in \sem{r'[n, \_]}$ respectively, \textit{i.e}, to $\sem{r}$. This, again, is a contradiction with our premise.

Altogether, this results in the fact that if there is no path $p \in \sem{\pt}$ from $(o_1, t_1)$ to $(o_2, t_2)$ then there is \textbf{no execution} that will return $\true$. Hence, we now proved that $\patheval(\Lthree)$ is in \pspace, which with the previous result implies \pspace-completeness.

==> z_t1.tex <==
\begin{figure*}[t]
    \begin{center}
        \resizebox{\textwidth}{!}{
        \begin{tikzpicture} 
            %%%%% node n1 
            \node[rect] (n1) {
                \alt{84pt}{ 
                    \urie{name} & \uriq{Ann}\\
                    \urie{school} & \uriq{MIT}
                }
            };
        
            %%%%% label of n1
            \node[rt] (ln1) at (n1.north) {
                \uri{$n_1$ $:$ Person}
            };
        
            %%%%% node n2
            \node[rect, right=2.6cm of n1] (n2) {
                \alt{66pt}{ 
                    \urie{name} & \uriq{Bob}
                }
            };
        
            %%%%% label of n2
            \node[rt] (ln2) at (n2.north) {
                \uri{$n_2$ $:$ Person}
            };
        
            %%%%% edge e1
            \draw[arr, bend left=10] (n1) to node[above, erect] (e1) {
                \alt{50pt}{
                    \urie{T} & \uritm{$[2,6]$}\\
                    \urie{T} & \uriq{$[2,6]$}
                }
            }
            (n2);
        
            %%%%% label of e1
            \node[ert] (le1) at (e1.north) {
                \uri{$e_1$ $:$ co-author}
            };
        
            %%%%% edge e2
            %\draw[arrout, bend right=10] (n1) to 
            %node[below, ert] (e2) {
            %   \uri{$e_2$ $:$ directs}
            %}
            %(n2);
        
            %%%%% node n3
            \node[rect, right=2.8cm of n2] (n3) {
                \alt{70pt}{
                    \urie{name} & \uriq{Cat}\\
                    \urie{school} & \uriq{MIT}
                }
            };
        
            %%%%% label of n3
            \node[rt] (ln3) at (n3.north) {
                \uri{$n_3$ $:$ Person}
            };
        
            %%%%% edge e3
            \draw[arrin] (n2) to node[above, erect] (e3) {
                \alt{50pt}{
                    \urie{role} & \uriq{Delilah}\\
                    \urie{ref} & \uriq{IMDb}
                }
            }
            (n3);
        
            %%%%% label of e3
            \node[ert] (le3) at (e3.north) {
                \uri{$e_3$ $:$ acts\_in}
            };
        
        \end{tikzpicture}
    }
    
    \end{center}
    \caption{\julia{Under construction} A temporal property graph that describes a collaboration network. \label{fig:t1}}
\end{figure*}


==> z_university.tex <==
\begin{figure*}[t]
    \begin{center}
        \resizebox{\textwidth}{!}{
        \begin{tikzpicture} 
            %%%%% node n1 
            \node[rect] (n1) {
                \alt{60pt}{ 
                    \urie{name} & 
                    \uriq{Ann}\\
                    \urie{school} & \uriq{MIT}\\
                    \urieb{time} & \uriq{[1,4]}
                }
            };
            \node[rect, below=0cm of n1] (n11) {
                \alt{60pt}{
                    \urie{name} & \uriq{Ann}\\
                    \urie{school} & \uriq{NYU}\\
                    \urieb{time} & \uriq{[5,9]}
                }
            };

            %%%%% label of n1
            \node[rt] (ln1) at (n1.north) {
                \uri{$n_1$ $:$ Professor}
            };
         
            %%%%% node n2
            \node[rect, right=2.6cm of n1] (n2) {
                \alt{60pt}{ 
                    \urie{name} & \uriq{Bob}\\
                    \urie{school} & \uriq{MIT}\\
                    \urieb{time} & \uriq{[1,9]}
                }
            };
            
            %%%%% label of n2
            \node[rt] (ln2) at (n2.north) {
                \uri{$n_2$ $:$ Professor}
            };
        
            %%%%% edge e1
            \draw[arrb, bend left=10] (n1) to node[above, erect] (e1) {
                \alt{50pt}{
                    \urie{proj} & \uriq{graphs}\\
                    \urie{paper} & \uriq{VLDB18}\\
                    \urieb{time} & \uriq{[2,3]}
                }
            }
            (n2);
        
            %%%%% label of e1
            \node[ert] (le1) at (e1.north) {
                \uri{$e_1$ $:$ co-authors}
            };
        
            %%%%% edge e2
            %\draw[arrout, bend right=10] (n1) to 
            %node[below, ert] (e2) {
            %   \uri{$e_2$ $:$ directs}
            %}
            %(n2);
        
            %%%%% node n3
            \node[rect, right=2.8cm of n2] (n3) {
                \alt{60pt}{
                    \urie{name} & \uriq{Cat}\\
                    \urie{school} & \uriq{MIT}\\
                    \urieb{time} & \uriq{[3,5]}
                }
            };
        
            %%%%% label of n3
            \node[rt] (ln3) at (n3.north) {
                \uri{$n_3$ $:$ Student}
            };
        
        
           %%%%% node n4
            \node[rect, right=2.8cm of n3] (n4) {
                \alt{60pt}{
                    \urie{name} & \uriq{Dan}\\
                    \urie{school} & \uriq{MIT}\\
                    \urieb{time} & \uriq{[3,4]}
                }
            };
            \node[rect, below=0cm of n4] (n41) {
                \alt{60pt}{
                    \urie{name} & \uriq{Dan}\\
                    \urie{school} & \uriq{CMU}\\
                    \urieb{time} & \uriq{[6,12]}
                }
            };
        
            %%%%% label of n4
            \node[rt] (ln4) at (n4.north) {
                \uri{$n_4$ $:$ Student}
            };
            
            %%%%% node n5
            \node[rect, below=2.8cm of n2] (n5) {
                \alt{60pt}{
                    \urie{name} & \uriq{Fan}\\
                    \urie{school} & \uriq{NYU}\\
                    \urieb{time} & \uriq{[5,6]}
                }
            };
            
            %%%%% label of n5
            \node[rt] (ln5) at (n5.north) {
                \uri{$n_5$ $:$ Student}
            };
            
            %%%%% node n6
            \node[rect, below=2.8cm of n3] (n6) {
                \alt{60pt}{
                    \urie{name} & \uriq{Eve}\\
                    \urie{school} & \uriq{CMU}\\
                    \urie{role} & \uriq{dean}\\
                    \urieb{time} & \uriq{[2,9]}
                }
            };
            
            %%%%% label of n6
            \node[rt] (ln6) at (n6.north) {
                \uri{$n_6$ $:$ Professor}
            };
        
            
            
            %%%%% edge e2
            \draw[arrout, bend left=10] (n2) to node[above, erect] (e2) {
                \alt{50pt}{
                    \urie{degree} & \uriq{PhD}\\
                    \urieb{time} & \uriq{[3,5]}
                }
            }
            (n3);
            
            %%%%% label of e2
            \node[ert] (le2) at (e2.north) {
                \uri{$e_2$ $:$ advises}
            };
            
             %%%%% edge e3
            \draw[arrout, bend left=10] (n3) to node[above, erect] (e3) {
                \alt{50pt}{
                    \urieb{time} & \uriq{[3,5]}
                }
            }
            (n4);
            
            %%%%% label of e3
            \node[ert] (le3) at (e3.north) {
                \uri{$e_3$ $:$ socializes}
            };
            
            %%%%% edge e4
            \draw[arrb, bend right=10] (n11) to node[below, erect] (e4) {
                \alt{50pt}{
                    \urie{paper} & \uriq{PODS19}\\
                    \urieb{time} & \uriq{[4,5]}
                }
            }
            (n2);
        
            %%%%% label of e4
            \node[ert] (le4) at (e4.north) {
                \uri{$e_4$ $:$ co-authors}
            };
            
             %%%%% edge e5
            \draw[arrb, bend right=10] (n2) to node[below, erect] (e5) {
                \alt{50pt}{
                    \urie{proj} & \uriq{XML}\\
                    \urie{paper} & \uriq{PODS16}\\
                    \urieb{time} & \uriq{[1,2]}
                }
            }
            (n3);
            
             %%%%% label of e5
            \node[ert] (le5) at (e5.north) {
                \uri{$e_5$ $:$ co-authors}
            };
        
        
           
            
          
            %%%%% edge e6
            \draw[arrout, bend right=15] (n11) to node[below, erect] (e6) {
                \alt{50pt}{
                    \urie{degree} & \uriq{MS}\\
                    \urieb{time} & \uriq{[5,6]}
                }
            }
            (n5);
            
            %%%%% label of e6
            \node[ert] (le6) at (e6.north) {
                \uri{$e_6$ $:$ advises}
            };
            
            %%%%% edge e7
            \draw[arrin, bend left=10] (n5) to node[below, erect] (e7) {
                \alt{50pt}{
                  \urie{hobby} & \uriq{dance}\\
                  \urieb{time} & \uriq{[5,6]}
                }
            }
            (n6);
            
            %%%%% label of e7
            \node[ert] (le7) at (e7.north) {
                \uri{$e_7$ $:$ socializes}
            };
            
            %%%%% edge e8
            \draw[arrout, bend right=15] (n6) to node[below, erect] (e8) {
                \alt{50pt}{
                    \urie{degree} & \uriq{MS}\\
                    \urieb{time} & \uriq{[6,7]}
                }
            }
            (n41);
            
            %%%%% label of e8
            \node[ert] (le8a) at (e8.north) {
                \uri{$e_8$ $:$ advises}
            };
            
            %%%%%
            \node[erect,below=0cm of e8] (le8b) {
                \alt{50pt}{
                    \urie{degree} & \uriq{PhD}\\
                    \urieb{time} & \uriq{[8,11]}
                }
            };
            
            
        \end{tikzpicture}
    }
    \end{center}
    \caption{A temporal property graph that describes students, professors, and their interactions in a university. \label{fig:uni}}
\end{figure*}

